Fast Algorithms for Segmented Regression

We study the fixed design segmented regression problem: Given noisy samples from a piecewise linear function $f$, we want to recover $f$ up to a desired accuracy in mean-squared error. Previous rigorous approaches for this problem rely on dynamic programming (DP) and, while sample efficient, have running time quadratic in the sample size. As our main contribution, we provide new sample near-linear time algorithms for the problem that -- while not being minimax optimal -- achieve a significantly better sample-time tradeoff on large datasets compared to the DP approach. Our experimental evaluation shows that, compared with the DP approach, our algorithms provide a convergence rate that is only off by a factor of $2$ to $4$, while achieving speedups of three orders of magnitude.

==> algorithm-full-backup.tex <==
\section{Finding the least squares estimator via DP}
In this section we first present a dynamic programming approach to piecewise linear regression.
We do not believe these results are fundamentally novel, however
to the best of our knowledge, these results appear primarily as folklore in the literature.
For completeness we demonstrate the fastest DP we are aware of, and we also prove its statistical guarantees.
This will serve as a warm-up for the later, more challenging proofs, and a similar result will be helpful in the later analyses.
\subsection{The exact DP}
We first describe how the exact DP works.
It simply outputs the least squares fit to the data amongst all 
$k$-piecewise linear functions, namely,
\[\arg \min_{f \in \mathcal{L}_k} \sum_{i = 1}^n \left(y_i - f(\vec{x}_i) \right)^2 \; .\]
It does this as follows.
For $i = 1, \ldots, n$ and $j = 1, \ldots, k$, let $A(i, j)$ denote the best error achievable by a $j$-piecewise linear function on the data pairs $\{ (\vec{x}_\ell, y_\ell) \}_{\ell = 1}^i$, that is, the best error achievable by $j$ pieces for the first $i$ data points.
Then it is not hard to see that 
\[A(i, j) = \min_{i' < i} \left( \mathrm{err} (\vec{X}, \vec{y}, \{i' + 1, \ldots, i \}) + A(i', j - 1) \right) \; , \]
where for any interval $I$, we have $ \mathrm{err} (\vec{X}, \vec{y}, I)$ denotes the sum-squared error to the data of the best linear least squares fit for the data points $\{ (\vec{x}_\ell, y_\ell) \}_{\ell \in I}$, that is, if $\fLS^I$ is the linear least squares fit to the data in $I$, then $ \mathrm{err} (\vec{X}, \vec{y}, I) = \sum_{\ell \in I} (y_i - \fLS^I (\vec{x}_i))^2$.

The algorithm then uses dynamic programming to fill out this $n \times k$ sized table of $A$ values, starting at $i = 1$ and $j = 1$, and then after having done so, it does one additional pass backwards over the table to find the path through the table that achieved the best error.
We can optimize this by first computing all of the $\mathrm{err} (\vec{X}, \vec{y}, \{i' + 1, \ldots, i \})$ for all $i' < i$, and then using a lookup table to find their values while actually executing the DP.
Given such a lookup table, the DP runs in time $O(n^2 k)$.
Naively, the construction of this look-up table would take time which is $O(n^3 d^2)$ since there are $O(n^2)$ linear regression problems, each of which take $O(n d^2)$ time to solve.

This run-time can be improved as follows. As mentioned above, if $\vec{A} \in \R^{n \times d}$ is a data matrix, and  $\vec{b}$ is a set of responses, then the least squares fit is of the form $\vec{A}^T \vec{A} \vec{z} = \vec{A}^T \vec{b}$.
Then, assuming the matrix $\vec{A}^T \vec{A}$ is invertible, we have that $\vec{z} = \left( \vec{A}^T \vec{A} \right)^{-1} \vec{A}^T \vec{b}$.
Moreover, the error of the fit is given by
\begin{align*}
\left\| \vec{A} \vec{z} - \vec{b} \right\|^2 &= \left( \vec{A} \vec{z} - \vec{b} \right)^T \left( \vec{A} \vec{z} - \vec{b} \right) \\
&= \vec{z}^T \vec{A}^T \vec{A} \vec{z} - 2 \vec{b}^T \vec{A} \vec{z} + \vec{b}^t \vec{b} \\
&= \vec{b}^T \vec{A} \left[ \left( \vec{A}^T \vec{A} \right) \right]^{-1} \vec{A}^T \vec{b} - 2 \vec{b}^T \vec{A} \vec{z} + \vec{b}^T \vec{b} \; .
\end{align*}
Now given $\left( \vec{A}^T \vec{A} \right)^{-1}$ and $\vec{A}^T \vec{b}$, we can compute all the remaining quantities in time $O(d^2)$.
To compute these quantities, we use the fact that our many regression instances are closely related, and we can reuse computations from previous regression instances to speed up future regression instances.

Concretely, the calculations above indicate that we need to compute $\left( \vec{X}^I \right)^T \vec{y}^I$ for all intervals $I \subseteq [n]$.
But these are all just sub-vectors of the vector $\vec{X}^T \vec{y}$, which we compute once in time $O(n d)$ and then use later on in all of the remaining computations.
Moreover, we also need to compute $\left( \left( \vec{X}^I \right)^T \vec{X}^I \right)^{-1}$ for all $I \subseteq [n]$.
However, observe that if we let $I = \{\ell, \ldots, p - 1\}$ for $\ell < p$, then $\left( \vec{X}^{I \cup \{p\}} \right)^T \vec{X}^{I \cup \{p\}} = \left( \vec{X}^I \right)^T \vec{X}^I + \vec{x}_p \vec{x}_p^T$. Therefore adding a single data point to the data matrix corresponds to a rank-one update of the data matrix.
Moreover, the effect of a rank-one update to the inverse of the matrix is well-known:
\begin{theorem}[Sherman-Morrison formula]
Suppose $\vec{M} \in \R^{d \times d}$ is an invertible square matrix, and let $\vec{v} \in \R^d$ be so that $1 + \vec{v}^T \vec{M}^{-1} \vec{v} \neq 0$.
Then
\[
\left( \vec{M} + \vec{v} \vec{v}^T \right)^{-1} = \vec{M}^{-1} - \frac{\vec{M}^{-1} \vec{v} \vec{v}^T \vec{M}^{-1}}{1 + \vec{v}^T \vec{M}^{-1} \vec{v}} \; .
\]
Thus, given $\vec{M}^{-1}$ and $\vec{v}$ satisfying these conditions, we may compute $\left( \vec{M} + \vec{v} \vec{v}^T \right)^{-1}$ in time $O(d^2)$.
\end{theorem}
Therefore, the dynamic program can do as follows: for each $\ell = 1, \ldots, n$, first compute $\left( \left( \vec{X}^I \right)^T \vec{X}^I \right)^{-1}$ for the interval $I$ of length $d$ starting at $\ell$, and then use the Sherman-Morrison update formula\footnote{In general, our matrices may not be invertible, or the update vector may not satisfy the condition in the Sherman-Morrison formula, but in practice it seems these issues don't come up and thus we do not worry about them here.
In general there are more complicated formulas for rank one updates for pseudo-inverses here but we will not cover them for simplicity.} 
to compute $\left( \left( \vec{X}^I \right)^T \vec{X}^I \right)^{-1}$ for every interval $I$ starting at $\ell$ in total time $O(n d^2)$.
Thus the algorithm takes $O(n^2 d^2)$ time to compute all of the $\left( \left( \vec{X}^I \right)^T \vec{X}^I \right)^{-1}$.
Combining the run-times we obtain the following run-time result for the dynamic program. 
\begin{theorem}
\label{thm:time-DP}
The exact dynamic program runs in time $O(n^2 (d^2 + k))$.
\end{theorem}
\subsection{Error analysis for the exact DP}
We now turn our attention to the learning rate of the exact DP.
We show:
\begin{theorem}
\label{thm:DP}
Let $\delta > 0$, and let $\fLS$ be the $k$-piecewise linear estimator returned by the exact DP.
Then, with probability at least $1 - \delta$,
\[\MSE (\fLS) \; \leq \; O\left(\sigma^2 \, \frac{kr + k \log \frac{n}{\delta}}{n}\right) \; .\]
\end{theorem}
\begin{proof}
We follow the proof technique for convergence of linear least squares as presented in~\cite{Rigollet15}. \todo{find right citation. Ludwig: I guess Philippe's notes are OK?}
Recall that $f$ is the true $k$-piecewise linear function.
By definition of least squares fit, we have 
=======
We follow the proof technique for convergence of linear least squares as presented in \cite{Rig15}.
Recall $f$ is the true $k$-piecewise linear function.
Then, by the definition of the least squares fit, we have that
\begin{align*}
\sum_{i = 1}^n (y_i - \fLS(\vec{x}_i))^2 &\leq \sum_{i = 1}^n (y_i - f(\vec{x}_i))^2 \\
&= \sum_{i = 1}^n \epsilon_i^2 \; .
\end{align*}
By expanding out the LHS, we have that
\begin{align*}
\sum_{i = 1}^n (y_i - \fLS(\vec{x}_i))^2 \; &= \; \sum_{i = 1}^n ( f(\vec{x}_i) + \epsilon_i - \fLS(\vec{x}_i))^2 \\
&= \; \sum_{i = 1}^n (\fLS (\vec{x}_i) - f(\vec{x}_i))^2 + 2 \sum_{i = 1}^n \epsilon_i (f(\vec{x}_i) - \fLS(\vec{x}_i)) + \sum_{i = 1}^n \epsilon_i^2 \ . \numberthis \label{eq:DP-LHS}
\end{align*}
Combining these two equations, with probability at least $1-\delta$, 
\begin{align*}
\sum_{i = 1}^n (\fLS (\vec{x}_i) - f(\vec{x}_i))^2 \; &\leq \; 2 \sum_{i = 1}^n \epsilon_i (\fLS(\vec{x}_i) - f(\vec{x}_i)) \\
&\leq \; O \left( \sigma \sqrt{kr + k \log \frac{n}{\delta}} \right) \cdot \| \vec{\fLS} - \vec{f} \| \; ,
\end{align*}
where the last equation follows from Corollary \ref{cor:sim-incoherence}.
A simple algebraic manipulation  from this last inequality yields the desired statement.
\end{proof}

<<<<<<< HEAD
The same proof technique can also be  adapted to show the following extension of Theorem \ref{thm:DP}:\todo{still not sure where we should put this lemma}
=======
The same proof technique can also be easily adapted to show the following, slight extension of Theorem \ref{thm:DP}:
>>>>>>> a0a8f265ed05559eb66e879686002d9a33d34dc0
\begin{lemma}
\label{lem:flat}
Fix $\delta > 0$.
Then with probability $1 - \delta$ we have that for all disjoint sets of $k$ intervals $J_1, \ldots, J_k$ of $[n]$ so that $f$ is flat on each $J_\ell$, the following inequality holds:
\[
  \sum_{\ell = 1}^k \sum_{i \in J_\ell} (\fLS^{J_\ell} (\vec{x}_i) - f(\vec{x}_i))^2 \; \leq \; O (\sigma^2 \, k (r + \log (n / \delta))) \; .
\]
\end{lemma}

\section{A simple greedy merging algorithm}
In this section, we propose a novel greedy algorithm that runs much faster than the DP, but which achieves a somewhat worse learning rate.
However, we show both theoretically and experimentally that the tradeoff between speed and statistical accuracy for this algorithm is markedly better than that achieved by the exact DP.

\subsection{The greedy merging algorithm}
<<<<<<< HEAD
The overall structure of the algorithm is quite similar to \cite{ADHLS15}, however, the merging criterion is different, and as explained above, the guarantees proved in that paper are insufficient to give non-trivial learning guarantees for regression. \todo{make sure this is done somewhere}
=======
The overall structure of the algorithm is quite similar to \cite{ADHLS15}, however, the merging criterion is different, and as explained above, the guarantees proved in that paper are insufficient to give non-trivial learning guarantees for regression.
>>>>>>> a0a8f265ed05559eb66e879686002d9a33d34dc0

Our algorithm requires the knowledge of $s^2$, the variance of the $\epsilon_i$'s, i.e. $s^2 = \EE [\epsilon_i^2]$.
We observe that $s^2$ guaranteed to be finite since $\epsilon_i$ are sub-Gaussian.
It is in general not equal to the variance proxy $\sigma^2$, however, it is well-known that $s^2 \leq \sigma^2$.
Requiring that we know $s^2$ is a drawback, and in Section \ref{sec:bucketing} we give a slightly more complicated algorithm which does not require knowledge of $s$.

We give the formal pseudocode for the algorithm in Algorithm \ref{alg:greedy}.
In the pseudocode we provide two additional tuning parameters $\tau, \gamma$.
This is because in general our algorithm cannot provide a $k$-histogram, but instead provides an $O(k)$ histogram, which for most practical applications suffices.
The tuning parameters allow us to trade off running time for fewer pieces.
In the typical use case we will have $\tau, \gamma = \Theta(1)$, in which case our algorithm will output an $O(k)$-piecewise linear function in time $O(n d^2 \log n)$ time.

\begin{algorithm*}[htb]
\begin{algorithmic}[1]
\Function{GreedyMerging}{$\tau, \gamma, s, \vec{X}, \vec{y}$}

\LineComment{\emph{Initial partition of $[n]$ into intervals of length $1$.}}
\State $\setI^0 \gets \{\{ 1 \}, \{ 2 \}, \ldots, \{ n \}\}$ 
%\vspace{.2cm}

\LineComment{\emph{Iterative greedy merging (we start with $j \gets 0$).}}
%\State $j \gets 0$
\While{$| \setI^j | > (2 + \frac{2}{\tau}) k + \gamma$}
  \State Let $s_j$ be the current number of intervals.
  %\vspace{.2cm}
  \LineComment{\emph{Compute the least squares fit and its error for merging neighboring pairs of intervals.}}
  \For{$u \in \{1, 2, \ldots, \frac{s_j}{2}\}$}
    \State $\theta_u \gets \textsc{LeastSquares}(\vec{X}, \vec{y}, I_{2u - 1} \cup I_{2u})$
    \State $e_u = \| \vec{y}^I - \vec{X}^I \theta_u \|_2^2 - s^2 |I_{2u - 1} \cup I_{2u}|$
  \EndFor
  \State Let $L$ be the set of indices $u$ with the $(1 + \frac{1}{\tau})k$ largest errors $e_u$, breaking ties arbitrarily. \label{line:L}
  \State Let $M$ be the set of the remaining indices. 
  %\vspace{.2cm}
  %\LineComment{Keep the intervals with the large merging errors.}
  \LineComment{\emph{Keep the intervals with large merging errors.}}
  \State $\setI^{j+1} \gets \bigcup\limits_{u \in L} \{I_{2u - 1}, I_{2u}\}$ 
  %\LineComment{Merge the remaining intervals.}
  \LineComment{\emph{Merge the remaining intervals.}}
  \State $\setI^{j+1} \gets \setI^{j+1} \cup \{I_{2u - 1} \cup I_{2u} \, | \, u \in M \}$ 
  %\vspace{.2cm}
  \State $j \gets j + 1$
\EndWhile
%\vspace{.2cm}
\State \textbf{return} the least squares fit to the data on every interval in $\setI^j$

\EndFunction
\end{algorithmic}
\caption{Piecewise linear regression by greedy merging.}
\label{alg:greedy}
\end{algorithm*}

\subsection{Runtime of \textsc{GreedyMerging}}
In this section we prove that our algorithm has the following, nearly-linear running time.
The analysis is similar to the analysis presented in \cite{ADHLS15}.
\begin{theorem}
\label{thm:time-greedy}
Let $\vec{X}$ and $\vec{y}$ be as above. Then $\textsc{GreedyMerging}(\tau, \gamma, s, \vec{X}, \vec{y})$ outputs a $\left( (2 + \frac{2}{\tau}) k + \gamma \right)$-piecewise linear function and runs in time $O(nd^2 \log(n / \gamma))$.
\end{theorem}
Before we prove this theorem, we compare this with the running time for the exact DP as given in Theorem \ref{thm:time-DP}.
Our main advantage is that our runtime scales linearly with $n$ instead of quadratically. This manifests itself as a substantially win theoretically in most reasonable regimes, and also as a big win in practice---see our experiments for more details there.
 
\begin{proof}[Proof of Theorem \ref{thm:time-greedy}]
We first bound the time it takes to run any single iteration of the algorithm.
In any iteration $j$, we do a linear least squares regression problem on each interval $I \in \setI^j$; each such problem takes $O(|I| d^2)$ time; hence solving them all takes $O(n d^2)$ time.
Computing the $e_u$ given the least squares fit takes no additional time asymptotically,
and finding the $\left( 1 + \frac{1}{\tau}\right)$ largest errors takes linear time \cite{CLRS09}.
Afterwards the remaining computations in this iteration can easily be seen to be done in linear time.
Hence each iteration takes $O(n d^2)$ time to complete.

We now bound the number of iterations of the algorithm.
By the same analysis as that done in the proof of Theorem 3.4 in \cite{ADHLS15} one can show that the algorithm terminates after at most $\log (n / \gamma)$ iterations.
Thus the whole algorithm runs in time $O(nd^2 \log(n / \gamma))$ time, as claimed.
\end{proof}

\subsection{Analysis of \textsc{GreedyMerging}}

\begin{theorem}
\label{thm:greedy}
Let $\delta > 0$, and let $\fhat$ be the estimator returned by \textsc{GreedyMerging}.
Let $m = (2 + \frac{2}{\tau}) k + \gamma$ be the number of pieces in $\fhat$.
Then, with probability $1 - \delta$, we have that
\[\MSE (\fhat) \leq O\left( \sigma^2 \left( \frac{m (r + \log (n / \delta) )}{n} \right) + \sigma \frac{\tau + \sqrt{k}}{\sqrt{n}} \log \left( \frac{n}{\delta} \right) \right) \; .\]
\end{theorem}


\begin{proof}
We first condition on the event that Corollaries \ref{cor:unif-err-bound}, \ref{cor:int-incoherence} and \ref{cor:sim-incoherence}, and Lemma \ref{lem:flat} all hold with error parameter $O(\delta)$, so that together they all hold with probability at least $1 - \delta$.
Let $\setI = \{ I_1, \ldots, I_{m} \}$ be the final partition of $[n]$ that our algorithm produces.
Recall $f$ is the ground truth $k$-piecewise linear function.
We partition the intervals in $\setI$ into two sets:  
\begin{align*}
\mathcal{F} &= \{I \in \setI: \mbox{$f$ is flat on $I$} \} \; ,\\
\mathcal{J} &= \{I \in \setI: \mbox{$f$ has a jump on $I$} \; .
\end{align*}
We first bound the error over the intervals in $\mathcal{F}$.
By Lemma \ref{lem:flat}, we have
\begin{equation}
\label{eq:flat}
\sum_{I \in \mathcal{F}} \sum_{i \in I} (f(\vec{x}_i) - \fhat (\vec{x}_i))^2 \; \leq \; O (\sigma^2 |\mathcal{F}| (r + \log ( n / \delta))) \;,
\end{equation}
with probability at least $1 - O(\delta)$.

We now turn our attention to the intervals in $\mathcal{J}$ and distinguish two further cases.
We let $\mathcal{J}_1$ be the set of intervals in $\mathcal{J}$ which were never merged, and we let $\mathcal{J}_2$ be the remaining intervals.
If the interval $I \in \mathcal{J}_1$ was never merged, the interval contains $1$ point $i$.
Because we may assume that $\vec{x}_i$, we know that for this one point, our estimator satisfies $\fhat (\vec{x}_i) = y_i$, since this is clearly the least squares fit for a linear estimator on $1$ nonzero point.
Hence Corollary \ref{cor:unif-err-bound} implies that the following inequality holds with probability at least $1 - O(\delta)$:
\begin{align*}
\sum_{I \in \mathcal{J}_1} \sum_{i \in I} (f(\vec{x}_i) - \fhat (\vec{x}_i))^2 &= \sum_{I \in \mathcal{J}_1} \sum_{i \in I} \epsilon_i^2 \\
&\leq \sigma^2 \left( \sum_{I \in \mathcal{J}_1} |I| + O \left( \log \frac{n}{\delta} \right) \sqrt{\sum_{I \in \mathcal{J}_1} 1} \right) \\
&\leq \sigma^2 \left( m + O \left( \log \frac{n}{\delta} \right) \sqrt{m} \right) \; . \numberthis \label{eq:jump1}
\end{align*}

We now finally turn our attention to the intervals in $\mathcal{J}_2$.
Fix $I \in \mathcal{J}_2$.
By definition, it was merged in some iteration of the algorithm.
This implies that in that iteration, there were $(1 + 1 / \tau) k$ intervals $M_1, \ldots, M_{(1 + 1/ \tau) k}$ so that for each interval $M_\ell$, we have
\begin{equation}
\label{eq:merge-cond}
\sum_{i \in I} (y_i - \fhat(\vec{x}_i))^2 - s^2 |I| \; \leq \; \sum_{i \in M_\ell} (y_i - \fLS^{M_\ell} (\vec{x}_i) )^2 - s^2 |M_\ell| \; .
\end{equation}
Since the true, underlying $k$-piecewise linear function $f$ has at most $k$ jumps, this means that there are at least $k / \tau$ of the $M_\ell$ on which $f$ is continuous.
WLOG assume that these are $M_1, \ldots, M_{k / \tau}$.

Fix any $\ell = 1, \ldots, k / \tau$.
Expanding out the RHS of Equation \ref{eq:merge-cond} using the definition of $y_i$ gives
\begin{align*}
\sum_{i \in M_\ell} (y_i - \fLS^{M_\ell} (\vec{x}_i))^2 - s^2 |M_\ell| &= \sum_{i \in M_\ell} \left[ (f(\vec{x}_i) - \fLS^{M_\ell} (\vec{x}_i))^2 + 2 \epsilon_i (f(\vec{x}_i) - \fLS^{M_\ell} (\vec{x}_i)) + \epsilon_i^2  \right] - s^2 |M_\ell| \\
&= \sum_{i \in M_\ell}  (f(\vec{x}_i) - \fLS^{M_\ell} (\vec{x}_i))^2 + 2 \sum_{i \in M_\ell} \epsilon_i (f(\vec{x}_i) - \fLS^{M_\ell} (\vec{x}_i)) + \sum_{i \in M_\ell} (\epsilon_i^2 - s^2) \; .
\end{align*}
Thus, we have that in aggregate,
\begin{align*}
\sum_{\ell = 1}^{k / \tau} \sum_{i \in M_\ell} (y_i - \fLS^{M_\ell} (\vec{x}_i))^2 - s^2 |M_\ell|& =  \sum_{\ell = 1}^{k / \tau} \sum_{i \in M_\ell}  (f(\vec{x}_i) - \fLS^{M_\ell} (\vec{x}_i))^2 \\
&+ 2 \sum_{\ell = 1}^{k / \tau} \sum_{i \in M_\ell} \epsilon_i (f(\vec{x}_i) - \fLS^{M_\ell} (\vec{x}_i)) + \sum_{\ell = 1}^{k / \tau}\sum_{i \in M_\ell} (\epsilon_i^2 - s^2) \; . \numberthis \label{eq:flat-allterms}
\end{align*}
We will upper bound each term on the RHS in turn.
First, since the function $f$ is continuous on each $M_\ell$ for $\ell = 1, \ldots, k / \tau$, Lemma \ref{lem:flat} implies
\begin{equation}
\label{eq:flat-term1}
\sum_{\ell = 1}^{k / \tau} \sum_{i \in M_\ell} (f(\vec{x}_i) - \fLS^{M_\ell} (\vec{x}_i))^2 \leq O \left(\sigma^2 \frac{k}{\tau} \left(r + \log \left( \frac{n}{\delta} \right) \right) \right) \; , \end{equation}
with probability at least $1 - O(\delta)$.

Moreover, note that the function $\fLS^{M_\ell}$ is a linear function on $M_\ell$ of the form $\fLS^{M_\ell}(\vec{x}) = \vec{x}^T \hat{\beta}$, where $\hat{\beta} \in \R^d$ is the least-squares fit on $M_{\ell}$.
Because $\vec{f}$ is just a fixed vector, the vector $\vec{f}^{M_\ell} -\vec{ \fLS}^{M_\ell} $ lives in the affine subspace of vectors of the form $\vec{f}^{M_\ell} + \vec{X}^{M_\ell} \eta$ where $\eta \in \R^d$ is arbitrary.
So Corollary \ref{cor:sim-incoherence} and Equation \ref{eq:flat-term1} imply that
\begin{align*}
\sum_{\ell = 1}^{k / \tau} \sum_{i \in M_\ell} \epsilon_i (f(\vec{x}_i) - \fLS^{M_\ell} (\vec{x}_i)) &\leq \sqrt{\sum_{\ell = 1}^{k / \tau}\sum_{i \in M_\ell} (f(\vec{x}_i) - \fLS^{M_\ell} (\vec{x}_i))^2} \cdot \sup_{\eta} \frac{|(\epsilon^{M_\ell})^T \vec{X} \eta |}{\| \vec{X} \eta \|} \\
&\leq O \left(\sigma^2 \frac{k}{\tau} \left(r + \log \left( \frac{n}{ \delta} \right) \right) \right)\; . \numberthis \label{eq:flat-term2}
\end{align*}
with probability $1 - O(\delta)$.

By Corollary \ref{cor:unif-err-bound}, we get that with probability $1 - O(\delta)$,
\[\sum_{\ell = 1}^{k / \tau} \left( \sum_{i \in M_\ell} \epsilon_i^2 - s^2 |M_\ell| \right) \leq O\left( \sigma \log \frac{n}{\delta} \right) \sqrt{n} \; .\]
Putting it all together, we get that
\begin{equation}
\label{eq:flat-term3} 
\sum_{i = 1}^{k / \tau} \left( \sum_{i \in M_\ell} (y_i - \fLS^{M_\ell} (\vec{x}_i) )^2 - s^2 |M_\ell| \right) \leq O \left(\frac{k}{\tau} \sigma^2 \left(r+ \log \left( \frac{n}{\delta} \right) \right) \right) + O\left(\sigma \log \frac{n}{\delta} \right) \sqrt{n} \;  
\end{equation}
with probability $1 - O(\delta)$.
Since the LHS of Equation \ref{eq:merge-cond} is bounded by each individual summand above, this implies that the LHS is also bounded by their average, which implies that
\begin{align*}
\sum_{i \in I} (y_i - \fhat(\vec{x}_i))^2 - s^2 |I|  &\leq \frac{\tau}{k} \sum_{i = 1}^{k / \tau} \left( \sum_{i \in M_\ell} (y_i - \fLS^{M_\ell} (\vec{x}_i) )^2 - s^2 |M_\ell| \right) \\
&\leq  O \left(\sigma^2 \left(r + \log \left( \frac{n}{\delta} \right) \right) \right) + O\left(\sigma \log \frac{n}{\delta} \right) \frac{\tau \sqrt{n}}{k} \; . \numberthis \label{eq:upper-bound}
\end{align*}
We now similarly expand out the LHS of Equation \ref{eq:merge-cond}:
\begin{align*}
\sum_{i \in I} (y_i - \fhat(\vec{x}_i))^2 - s^2 |I| &= \sum_{i \in I} (f (\vec{x}_i) + \epsilon_i - \fhat(\vec{x}_i))^2 - s^2 I \\
&= \sum_{i \in I} (f (\vec{x}_i) - \fhat (\vec{x}_i))^2 + 2 \sum_{i \in I} \epsilon_i (f (\vec{x}_i) - \fhat (\vec{x}_i)) + \sum_{i \in I} \left( \epsilon_i^2 - s^2 \right) \numberthis \label{eq:jump-allterms}
\end{align*}
From this we are interested in obtaining an upper bound on $\sum_{i \in I} (f (\vec{x}_i) - \fhat (\vec{x}_i))^2$, hence we seek to lower bound the second and third terms of Equation \ref{eq:jump-allterms}.
The calculations here will very closely mirror those done above.

By Corollary \ref{cor:int-incoherence}, we have that
\[ 
2 \sum_{i \in I} \epsilon_i (f (\vec{x}_i) - \fhat (\vec{x}_i)) \geq - O \left(\sigma \sqrt{r + \log \left( \frac{n}{\delta} \right)} \right) \sqrt{\sum_{i \in I} (f (\vec{x}_i) - \fhat (\vec{x}_i))^2} \; ,
\]
and by Corollary \ref{cor:unif-err-bound} we have
\[
 \sum_{i \in I} \left( \epsilon_i^2 - s^2 \right) \geq - O \left(\sigma \log \frac{n}{\delta} \right) \sqrt{|I|} \; ,
\]
and so
\begin{align*}
\sum_{i \in I} (y_i - \fhat(\vec{x}_i))^2 - s^2 |I| &\geq \sum_{i \in I} (f(\vec{x}_i) - \fhat(\vec{x}_i))^2 \\
&- O \left(\sigma \sqrt{r + \log \left( \frac{n}{\delta} \right)} \right) \sqrt{\sum_{i \in I} (f (\vec{x}_i) - \fhat (\vec{x}_i))^2} - O \left(\sigma \log \frac{n}{\delta} \right) \sqrt{|I|} \; . \numberthis \label{eq:lower-bound}
\end{align*}
Putting Equations \ref{eq:upper-bound} and \ref{eq:lower-bound} together yields that with probability $1 - O(\delta)$,
\begin{align*}
\sum_{i \in I} (f(\vec{x}_i) - \fhat(\vec{x}_i))^2 &\leq O \left( \sigma^2 \left(r + \log \left( \frac{n}{\delta} \right) \right) \right) \\
&+ O \left(\sigma \sqrt{r + \log \left( \frac{n}{\delta} \right)} \right) \sqrt{\sum_{i \in I} (f (\vec{x}_i) - \fhat (\vec{x}_i))^2} + O\left( \sigma \log \frac{n}{\delta} \right) \left( \frac{\tau \sqrt{n}}{k} + \sqrt{|I|} \right) \; .
\end{align*}

Letting $x^2 = \sum_{i \in I} (\fhat (\vec{x}_i) - f(\vec{x}_i))^2$, then this inequality is of the form $x^2 \leq b x + c$ where $b, c \geq 0$.
In this specific case, we have that
\begin{align*}
b &= O \left( \sigma \sqrt{r + \log \frac{n}{\delta} } \right) \; ,~ \mbox{and} \\
c &= O \left( \sigma^2 \left(r + \log \left( \frac{n}{\delta} \right) \right) \right) + O\left( \sigma \log \frac{n}{\delta} \right) \left( \frac{\tau \sqrt{n}}{k} + \sqrt{|I|} \right)
\end{align*}
We now prove the following lemma about the behavior of such inequalities:
\begin{lemma}
\label{lem:quadratic}
Suppose $x^2 \leq bx + c$ where $b, c \geq 0$.
Then $x^2 \leq O(b^2 + c)$.
\end{lemma}
\begin{proof}
From the quadratic formula, the inequality implies that $x \leq \frac{b + \sqrt{b + 4c}}{2}$.
From this, it is straightforward to demonstrate the desired claim.
\end{proof}
Thus, from the lemma, we have
\[
\sum_{i \in I} (f(\vec{x}_i) - \fhat(\vec{x}_i))^2 \leq O \left( \sigma^2 \left(r + \log \left( \frac{n}{\delta} \right) \right) \right) + O\left( \sigma \log \frac{n}{\delta} \right) \left( \frac{\tau \sqrt{n}}{k} + \sqrt{|I|} \right) \; .
\]

Hence the total error over all intervals in $\mathcal{J}_2$ can be bounded by:
\begin{align*}
\sum_{I \in \mathcal{J}_2} \sum_{i \in I} (f(\vec{x}_i) - \fhat(\vec{x}_i))^2 &\leq O \left(k \sigma^2 \left(r + \log \left( \frac{n}{\delta} \right) \right) \right) + O\left( \sigma \log \frac{n}{\delta} \right) \left( \tau \sqrt{n} + \sum_{I \in \mathcal{J}}\sqrt{|I|} \right) \\
&\leq O \left( k \sigma^2 \left(r + \log \left( \frac{n}{\delta'} \right) \right) \right) + O\left(\sigma \log \frac{n}{\delta} \right) \left( \tau \sqrt{n} + \sqrt{k n} \right) \numberthis \label{eq:jump2} \; .
\end{align*}
In the last line we use that the intervals $I \in \mathcal{J}_2$ are disjoint (and hence their cardinalities sum up to at most $n$), and that there are at most $k$ intervals in $\mathcal{J}_2$ because the function $f$ is $k$-piecewise linear.
Finally, applying a union bound and summing Equations \ref{eq:flat}, \ref{eq:jump1}, and \ref{eq:jump2} yields the desired conclusion.
\end{proof}

\section{A variance-free merging algorithm}
\label{sec:bucketing}
In this section we give a variant of the above algorithm which does not require the algorithm to know $s^2$.
The formal algorithm is given in Algorithm \ref{alg:bucket}.

\begin{algorithm*}[htb]
\begin{algorithmic}[1]
\Function{BucketGreedyMerging}{$\gamma, \vec{X}, \vec{y}$}

\LineComment{Initial histogram.}
\State Let $\setI^0 \gets \{\{ 1 \}, \{ 2 \}, \ldots, \{ n \}\}$ be the initial partition of $[n]$ into intervals of length $r$.
%\vspace{.2cm}

\LineComment{Iterative greedy merging (we start with $j = 0$).}
%\State $j \gets 0$
\While{$| \setI^j | > (2(k + 1) + \gamma) \log n$}
  \State Let $s_j$ be the current number of intervals.
  %\vspace{.2cm}
  \LineComment{Compute the least squares fit and its error for merging neighboring pairs of intervals.}
  \For{$u \in \{1, 2, \ldots, \frac{s_j}{2}\}$}
     \State $I'_u \gets I_{2u - 1} \cup I_{2u}$
    \State $\theta_u \gets \textsc{LeastSquares}(\vec{X}, \vec{y}, I'_u)$
    \State $e_u = \frac{1}{|I'_u|} \| \vec{y}^I - \vec{X}^I \theta_u \|_2^2 $
  \EndFor
  \For{$\alpha = 0, \ldots, \log (n) - 1$}
  	\State Let $B_\alpha$ be the set of $u$ so that $2^\alpha \leq |I'_u| \leq 2^{\alpha + 1}$
	\State Let $L_\alpha$ be the set of $u \in B_\alpha$ with the $k + 1$ largest $e_u$ amongst $u \in B_\alpha$, breaking ties arbitrarily
	\State $M_\alpha$ be the set of the remaining $u$ in $B_\alpha$. \label{line:L}
  	%\vspace{.2cm}
  	%\LineComment{Keep the intervals with the large merging errors.}
  	\State $\setI^{j+1} \gets \bigcup\limits_{u \in L_\alpha} \{I_{2u - 1}, I_{2u}\}$ 
  	\LineComment{\emph{Keep the intervals in each $B_\alpha$ with large merging errors.}}
  	%\LineComment{Merge the remaining intervals.}
  	\State $\setI^{j+1} \gets \setI^{j+1} \cup \{I'_u \, | \, u \in M_\alpha \}$ 
  	\LineComment{\emph{Merge the remaining intervals in each $B_\alpha$.}}
  \EndFor
  %\vspace{.2cm}
  \State $j \gets j + 1$
\EndWhile
%\vspace{.2cm}
\State \textbf{return} the least squares fit to the data on every interval in $\setI^j$

\EndFunction
\end{algorithmic}
\caption{Variance-free greedy merging with bucketing.}
\label{alg:bucket}
\end{algorithm*}

We now state the running time for \textsc{BucketGreedyMerge}.
The runtime analysis for \textsc{BucketGreedyMerge} is almost identical to that of \textsc{GreedyMerge}; hence we omit its proof.
\begin{theorem}
\label{thm:time-bucket}
Let $\vec{X}$ and $\vec{y}$ be as above. Then $\textsc{BucketGreedyMerging}(\gamma, \vec{X}, \vec{y})$ outputs a $\left(2 (k + 1) + \gamma \right) \log n$-piecewise linear function and runs in time $O(nd^2 \log(n / \gamma))$.
\end{theorem}


\subsection{Analysis of \textsc{BucketGreedyMerge}}
This section is dedicated to the proof of the following theorem:
\begin{theorem}
\label{thm:bucket}
Let $\fhat$ be the $m$-piecewise linear function that is returned by \textsc{BucketGreedyMerge}, where $m = \left(2 (k + 1) + \gamma \right) \log n$.
Then, with probability $1 - \delta$, we have
\[\MSE (\fhat) \leq O\left( \sigma^2 \left( \frac{m(r  + \log (n / \delta) )}{n} \right) + \sigma \sqrt{\frac{k}{n}} \log \left( \frac{n}{\delta} \right) \right) \; .\]
\end{theorem}
\begin{proof}
As in the proof of Theorem \ref{thm:greedy}, we let $\mathcal{I}$ be the final partition of $[n]$ that our algorithm produces.
We also similarly condition on the event that Corollaries \ref{cor:unif-err-bound} and \ref{cor:sim-incoherence} and Lemma \ref{lem:flat}  all hold with parameter $O(\delta)$.
We again partition $\setI$ into two sets $\mathcal{F}$ and $\mathcal{J}$ as before, and further subdivide $\mathcal{J}$ into $\mathcal{J}_1$ and $\mathcal{J}_2$.
The error on $\mathcal{F}$ and $\mathcal{J}_1$ is the same as the error given in Equations \ref{eq:flat} and \ref{eq:jump1}.
The only difference is the error on intervals in $\mathcal{J}_2$.

Let $I \in \mathcal{J}_2$ be fixed.
By definition this means there was some iteration and a collection of some $k + 1$ disjoint intervals $M_1, \ldots, M_{k + 1}$ so that $|M_\ell| / 2 \leq |I| \leq 2 |M_\ell|$ and
\[\frac{1}{|I|} \sum_{i \in I} (y_i - \fhat(\vec{x}_i))^2 \leq \frac{1}{|M_\ell|} \sum_{i \in M_\ell} (y_i - \fLS^{M_\ell} (\vec{x}_i))^2\]
for all $\ell = 1, \ldots, k + 1$.
Since $f$ has at most $k$ discontinuities, this means that there is at least one $M_\ell$ so that $f$ is continuous on $M_\ell$.
WLOG assume that $f$ is continuous on $M_1$.
By the same kinds of calculations done in the proof of Theorem \ref{thm:greedy}, we have that with probability $1 - \delta$,
\[\sum_{i \in M_1} (y_i - \fLS^{M_\ell} (\vec{x}_i))^2 \leq  O \left( \sigma^2 ( r + \log (n / \delta) ) \right) + \sigma^2 |M_\ell| +  O(\sigma \log (n / \delta)) \sqrt{|M_\ell|} \]
and
\begin{align*}
\sum_{i \in I} (y_i - \fhat (\vec{x}_i))^2 &\geq  \sum_{i \in I} (f(\vec{x}_i) - \fhat (\vec{x}_i))^2 -  O \left( \sigma \sqrt{r + \log (n / \delta) } \right) \sqrt{ \sum_{i \in I} (y_i - \fhat (\vec{x}_i))^2} + \sigma^2 |I| \\
&- O(\sigma \log (n / \delta)) \sqrt{|I|} \; ,
\end{align*}
and putting these two equations together and rearranging, we have
\begin{align*}
\sum_{i \in I} (f(\vec{x}_i) - \fhat (\vec{x}_i))^2 &\leq O \left( \sigma^2 (r + \log (n / \delta) ) \right) + \sigma^2 \cdot O(\log (n / \delta)) \left( \frac{|I|}{\sqrt{|M_\ell|}} + \sqrt{|I|} \right) \\
&~~~~ + O \left( \sigma \sqrt{r + \log (n / \delta) } \right) \sqrt{ \sum_{i \in I} (y_i - \fhat (\vec{x}_i))^2}\\
&\leq  O \left( \sigma^2 (r+ \log (n / \delta) ) \right) + O\left( \sigma^2 \log (n / \delta) \sqrt{|I|} \right) \\
&~~~~ + O \left( \sigma \sqrt{r + \log (n / \delta) } \right) \sqrt{ \sum_{i \in I} (y_i - \fhat (\vec{x}_i))^2} \; ,
\end{align*}
where the last inequality used that $|M_\ell| \geq |I| / 2$.
By Lemma \ref{lem:quadratic}, this implies that
\[
\sum_{i \in I} (f(\vec{x}_i) - \fhat (\vec{x}_i))^2 \leq O \left( \sigma^2 (r+ \log (n / \delta) ) \right) + O\left( \sigma^2 \log (n / \delta) \sqrt{|I|} \right) \; .
\]
Since there are at most $k$ elements in $\mathcal{J}_2$, and they are all disjoint, this yields that
\begin{equation}
\label{eq:bucketjump}
\sum_{I \in \mathcal{J}_2} \sum_{i \in I} (f(\vec{x}_i) - \fhat (\vec{x}_i))^2 \leq O \left( k \sigma^2 \left( r + \log \frac{n}{\delta} \right) \right) + O\left( \sigma  \log \left( \frac{n}{\delta} \right) \sqrt{k n} \right)
\end{equation}
and putting this equation together with Equations \ref{eq:flat} and \ref{eq:jump1} yields the desired conclusion.
\end{proof}

\subsection{Postprocessing}
One unsatisfying aspect of \textsc{BucketGreedyMerge} is that it outputs $O(k \log n)$ pieces. 
Not only does this increase the size of the representation nontrivially when $n$ is large, but it also increases the error rate: it is the reason why the first term in the error rate given in Theorem \ref{thm:bucket} has an additional $\log n$ factor as opposed the rate in Theorem \ref{thm:greedy}.
In this section we give an efficient postprocessing procedure for \textsc{BucketGreedyMerge} which, when run on the output of \textsc{BucketGreedyMerge}, outputs an $O(k)$ histogram with the same rate as before.
In fact, the rate is slightly improved as we are able to remove the $\log n$ factor mentioned above.

The postprocessing algorithm \textsc{Postprocessing} takes as input a partition $\setI$ of $[n]$ of size $O(k \log n)$ and $k$. 
It does the follows: starting from the $O(k \log n)$ partition $\setI$, run the DP, but searching only on intervals with breakpoints amongst the breakpoints of $\setI$, to find the $2k + 1$ partition $\setI_p$ whose endpoints are also endpoints of $\setI$ which minimizes the sum squared error to the data.
The runtime analysis is exactly identical to that of the DP, with two exceptions: we only need to fill out a $O(k \log n) \times (2k + 1)$ size table (as compared to an $n \times k$ sized table), and because we are no longer doing rank one updates as we instead will be doing updates in large chunks, we cannot use the Sherman-Morrison trick to speed up the computation of the least-squares fits.
Hence, we obtain the following theorem:
\begin{theorem}
\label{thm:time-postprocessing}
Given a partition $\setI$ of $[n]$ into $O(k \log n)$ pieces, $\textsc{Postprocessing}(\setI, k)$ runs in time $\Otilde(k^3 d^2)$, and outputs a $(2k + 1)$-piecewise linear function, where the $\Otilde$ hides $\poly \log (n)$ factors.
\end{theorem}

We now turn to show that it still provides the same (in fact, slightly better) statistical guarantees as the original partition:
\begin{theorem}
\label{thm:postprocessing}
Fix $\delta > 0$.
Let $\fhat_p$ be the estimator output by \textsc{PostprocessedBucketGreedyMerge}.
Then, with probability $1 - \delta$, we have
\[
\MSE (\fhat_p) \leq O \left( \frac{k \sigma^2 \left( r + \log \frac{n}{\delta} \right)}{n} + \sigma  \log \left( \frac{n}{\delta} \right) \sqrt{\frac{k}{n}} \right)
 \; .\]
\end{theorem}
\begin{proof}
Let $\setI$ and $\mathcal{J}$ be as in the proof of Theorem \ref{thm:bucket}.
Let $\setI_p = \{J_1, \ldots, J_{2k + 1}\}$ be the intervals in the partition that we return.
We again condition on the event that Corollaries \ref{cor:unif-err-bound} and \ref{cor:sim-incoherence} and Lemma \ref{lem:flat} all hold with parameter $O(\delta)$.
The following will then all hold with probability $ 1- \delta$.

Define the partition $\mathcal{K}$ to be the partition which contains every interval in $\mathcal{J}$, and exactly one interval between any two non-consecutive intervals in $\mathcal{J}$, and let $g$ be the $(2k + 1)$-piecewise linear function which is the least squares fit to the data on each interval in $I \in \mathcal{K}$.
This is clearly a possible solution for the dynamic program, and therefore we have
\begin{align*}
\sum_{i = 1}^n (\fhat (\vec{x}_i) - y_i)^2 &\leq\sum_{i = 1}^n (g (\vec{x}_i) - y_i)^2 \\
&= \sum_{I \in \mathcal{K} \setminus \mathcal{J}} \sum_{i \in I} (g(\vec{x}_i) - y_i)^2 +\sum_{I \in \mathcal{J}}  \sum_{i \in I} (g(\vec{x}_i) - y_i)^2 \; . \numberthis \label{eq:postDP-opt}
\end{align*}
We will expand and then upper bound the RHS of Equation \ref{eq:postDP-opt}.
First, by the same kinds of calculations as those done in the proof of Theorem \ref{thm:greedy}, we have that
\[\sum_{I \in \mathcal{K} \setminus \mathcal{J}} \sum_{i \in I} (g(\vec{x}_i ) - y_i^2) \leq O \left( k \sigma^2 \left( r + \log \frac{n}{\delta} \right) \right) +  \sum_{I \in \mathcal{K} \setminus \mathcal{J}} \sum_{i \in I} \epsilon_i^2 \; \; ,\]
and from Equation \ref{eq:bucketjump} and Corollary \ref{cor:sim-incoherence} we have
\begin{align*}
\sum_{I \in \mathcal{J}}  \sum_{i \in I} (g(\vec{x}_i) - y_i)^2 &= \sum_{I \in \mathcal{J}}  \sum_{i \in I} (f(\vec{x}_i) + \epsilon_i - g(\vec{x}_i))^2 \\
&= \sum_{I \in \mathcal{J}}  \sum_{i \in I} (f(\vec{x}_i) - g(\vec{x}_i))^2 + \sum_{I \in \mathcal{J}}  \sum_{i \in I} \epsilon_i (f(\vec{x}_i)- g(\vec{x}_i)) + \sum_{I \in \mathcal{J}}  \sum_{i \in I} \epsilon_i^2 \\
&\leq O \left( k \sigma^2 \left( r + \log \frac{n}{\delta} \right) \right) + O\left( \sigma  \log \left( \frac{n}{\delta} \right) \sqrt{k n} \right) +  \sum_{I \in \mathcal{J}} \sum_{i \in I} \epsilon_i^2 \; ,
\end{align*}
so all together now we have
\[
\sum_{I \in \mathcal{K}} \sum_{i \in I} (g (\vec{x}_i) - y_i)^2 \leq O \left( k \sigma^2 \left( r + \log \frac{n}{\delta} \right) \right) + O\left( \sigma  \log \left( \frac{n}{\delta} \right) \sqrt{k n} \right) + \sum_{i = 1}^n \epsilon_i^2
\]
Moreover, by the same kinds of calculations, we can expand out the LHS of Equation \ref{eq:postDP-opt}:
\begin{align*}
\sum_{i = 1}^n (\fhat (\vec{x}_i) - y_i)^2 &\geq \sum_{i = 1}^n (\fhat (\vec{x}_i) - f(\vec{x}_i))^2 + \sum_{i = 1}^n \epsilon_i (\fhat (\vec{x}_i) - f(\vec{x}_i)) + \sum_{i = 1}^n \epsilon_i^2 \\
&\geq \sum_{i = 1}^n (\fhat (\vec{x}_i) - f(\vec{x}_i))^2 - O \left( \sqrt{k} \cdot \sigma \sqrt{r + \log \frac{n}{\delta} } \right) \left(  \sum_{i = 1}^n (\fhat (\vec{x}_i) - f(\vec{x}_i))^2 \right)^{1/2} + \sum_{i = 1}^n \epsilon_i^2
\end{align*}
and hence, combining, cancelling, and moving terms around, we get that
\begin{align*}
\sum_{i = 1}^n (\fhat (\vec{x}_i) - f(\vec{x}_i))^2 &\leq O \left( \sqrt{k} \cdot \sigma \sqrt{r + \log \frac{n}{\delta} } \right) \left[ 1 +  \left(  \sum_{i = 1}^n (\fhat (\vec{x}_i) - f(\vec{x}_i))^2 \right)^{1/2} \right] \\
&+ O\left( \sigma  \log \left( \frac{n}{\delta} \right) \sqrt{k n} \right) \; .
\end{align*}
By Lemma \ref{lem:quadratic}, this implies that
\[\sum_{i = 1}^n (\fhat (\vec{x}_i) - f(\vec{x}_i))^2 \leq O \left( k \sigma^2 \left( r + \log \frac{n}{\delta} \right) + \sigma  \log \left( \frac{n}{\delta} \right) \sqrt{k n} \right) \; ,\]
with probability $1 - \delta$, as claimed.
\end{proof}

We remark that \textsc{Postprocessing} can also be run on the output of \textsc{GreedyMerging} to decrease the number of pieces from $O(k)$ to $2k + 1$ if so desired.
The proof that it maintains similar statistical guarantees is almost identical to the one presented above.
\section{Obtaining Agnostic Guarantees}
\label{sec:agnostic}
In this section we demonstrate how to show agnostic guarantees for the algorithms in the previous sections.
Recall now $f$ is arbitrary, and $f^\ast$ is a $k$-piecewise linear function which obtains the best approximation in mean-squared error to $f$ amongst all $k$-piecewise linear functions.
For all $i = 1,\ldots, n$, define $\gamma_i = f(\vec{x}_i) - f^\ast (\vec{x}_i)$ to be the error at data point $i$ of the approximation, so that for all $i$, we have $y_i = f^\ast (\vec{x}_i) + \gamma_i + \epsilon_i$.
By definition, we have that $\sum_{i = 1}^n \gamma_i^2 = n \cdot \OPT_k$.

As a warm-up, we first show the following agnostic guarantee for the exact DP:
\begin{theorem}
\label{thm:DP-agnostic}
Fix $\delta > 0$.
Let $\fLS$ be the $k$-piecewise linear function returned by the exact DP.
Then, with probability $1 - \delta$, we have 
\[
\MSE (\fLS) \leq O \left( \sigma^2 \frac{kr + k \log \frac{n}{\delta}}{n} + \sigma \log \left( \frac{1}{\delta} \right) \sqrt{\frac{\OPT_k}{n}} + \OPT_k \right)
\]
\end{theorem}
The middle term here looks strange---but is sufficiently small so that qualitatively in the regimes that are most interesting, i.e., when $\OPT_k$ is small, does not contribute meaningfully.
\begin{proof}
The overall proof structure stays the same.
From the definition of the least-squares fit, we have
\begin{align*}
\sum_{i = 1}^n (y_i - \fLS(\vec{x}_i))^2 &\leq \sum_{i = 1}^n (y_i - f^\ast(\vec{x}_i))^2 \\
&= \sum_{i = 1}^n (\epsilon_i + \gamma_i)^2 \\
&= \sum_{i = 1}^n \epsilon_i^2 + 2 \sum_{i = 1}^n \epsilon_i \gamma_i + n \cdot \OPT_k \\
&\leq \sum_{i = 1}^n \epsilon_i^2 + O \left( \sigma \log \frac{1}{\delta} \right) \left( n \cdot \OPT_k \right)^{1/2} + n \cdot \OPT_k \; ,
\end{align*}
with probability $1 - O(\delta)$, where the last inequality follows from the $r = 1$ case of Lemma \ref{lem:incoherence}.
The LHS can be expanded out exactly as before in Equation \ref{eq:DP-LHS}, and putting these two sides together we obtain that
\begin{align*}
\sum_{i = 1}^n (\fLS (\vec{x}_i) - f(\vec{x}_i))^2 \; &\leq \; 2 \sum_{i = 1}^n \epsilon_i (\fLS(\vec{x}_i) - f(\vec{x}_i)) + O \left(\sigma \log \frac{1}{\delta} \right) \left( n \cdot \OPT_k \right)^{1/2} + n \cdot \OPT_k\\
&\leq O \left( \sigma \sqrt{kr + k \log \frac{n}{\delta}} \right) \cdot \| \vec{\fLS} - \vec{f} \| + O \left(  \sigma \log \frac{1}{\delta} \right) \left( n \cdot \OPT_k \right)^{1/2} + n \cdot \OPT_k
\end{align*}
with probability at least $1 - O(\delta)$ and so by Lemma \ref{lem:quadratic} we obtain that
\[
\sum_{i = 1}^n (\fLS (\vec{x}_i) - f(\vec{x}_i))^2 \leq O \left( \sigma^2 \left( kr + k \log \frac{n}{\delta}\right) + \sigma \log \left( \frac{1}{\delta} \right) \left( n \cdot \OPT_k \right)^{1/2} + n \cdot \OPT_k \right) \;.
\]
Dividing both sides by $n$ yields the desired conclusion.
\end{proof}
Reviewing the proof, we observe the following general pattern: all upper bounds we wish to obtain (generally for formulas which occur on the RHS of the equations above) we obtain these new $\OPT_k$ factors, whereas the lower bounds (generally for formulas on the LHS of the equations above) nothing changes.
In fact all the proofs will follow this pattern.
We first establish some useful concentration bounds.
First, by the same union-bound technique used throughout this paper, one can show:
\begin{lemma}
\label{lem:agnostic-incoherence}
Fix $\delta > 0.$
Let $\epsilon_i$ and $\gamma_i$ be as above for $i = 1, \ldots, n$.
Then, with probability $1 - \delta$, we have that for all collections of $k$ disjoint intervals $J_1, \ldots, J_k$, the following holds:
\begin{align*}
\sum_{\ell = 1}^k \sum_{i \in J_\ell} \epsilon_i \gamma_i &\leq O \left( k \sigma \log \frac{n}{\delta} \right) \cdot \left( \sum_{\ell = 1}^k \sum_{i \in J_\ell} \gamma_i^2 \right)^{1/2} \\
&\leq O \left( k \sigma \log \frac{n}{\delta} \right) \cdot \left( n \cdot \OPT_k \right)^{1/2}
\end{align*}
\end{lemma}

Observe that with this Lemma, we can easily adapt the proof of Theorem \ref{thm:DP-agnostic} to show the following agnostic version of Lemma \ref{lem:flat}:
\begin{lemma}
\label{lem:agnostic-flat}
Fix $\delta > 0$. Then with probability $1 - \delta$ we have that for all disjoint sets of $k$ intervals $J_1, \ldots, J_k$ of $[n]$ so that $f^\ast$ is flat on each $J_\ell$, the following inequality holds:
\[
\sum_{\ell = 1}^k \sum_{i \in J_\ell} (\fLS^{J_\ell} (\vec{x}_i) - f(\vec{x}_i))^2 \leq O \left( \sigma^2 \left( kr + k \log \frac{n}{\delta}\right) + k \sigma \log \left( \frac{n}{\delta} \right) \left( n \cdot \OPT_k \right)^{1/2} + n \cdot \OPT_k \right) \; .
\]
\end{lemma}

With this lemma, we can now show the following theorem for our greedy algorithm, which shows that in the presence of model misspecification, our algorithm still performs at a good rate:
\begin{theorem}
Let $\delta > 0$, and let $\fhat$ be the estimator returned by \textsc{GreedyMerging}.
Let $m = (2 + \frac{2}{\tau}) k + \gamma$ be the number of pieces in $\fhat$.
Then, with probability $1 - \delta$, we have that
\[\MSE (\fhat) \leq O\left( \sigma^2 \left( \frac{m (r + \log (n / \delta)) }{n} \right) + \sigma \frac{\tau + \sqrt{k}}{\sqrt{n}} \log \left( \frac{n}{\delta} \right) + k \sigma \log \left( \frac{n}{\delta} \right) \sqrt{\frac{\OPT_k }{n}} + \tau \cdot \OPT_k \right) \; .\]
\end{theorem}
\begin{proof}
As before, we condition on the event that Corollaries \ref{cor:unif-err-bound}, \ref{cor:int-incoherence} and \ref{cor:sim-incoherence}, and Lemmas \ref{lem:agnostic-incoherence} and \ref{lem:agnostic-flat} all hold with error parameter $O(\delta)$, so that together they all hold with probability at least $1 - \delta$.
We also let $\setI, \mathcal{F}, \mathcal{J}_1,$ and $\mathcal{J}_2$ also denote the same quantities as before, except we define the partition with respect to the jumps of $f^\ast$ instead of $f$, since the latter would not make sense.
For instance, $\mathcal{F}$ is the set of intervals in $\setI$ on which $f^\ast$ has no jumps.

We again bound the error on these three sets separately.
First, by Lemma \ref{lem:agnostic-flat} we have that
\begin{equation}
\label{eq:-agnostic-flat}
\sum_{I \in \mathcal{F}} \sum_{i \in I} (f(\vec{x}_i) - \fhat (\vec{x}_i))^2 \; \leq \; O \left( \sigma^2 \left( mr + m \log \frac{n}{\delta}\right) + m \sigma \log \left( \frac{n}{\delta} \right) \left( n \cdot \OPT_k \right)^{1/2} + n \cdot \OPT_k \right) \; .
\end{equation}

Second, we bound the error on $\mathcal{J}_1$.
By the modifying the calculations as those preceding Equation \ref{eq:jump1} in the same way as we did above in the proof of Theorem \ref{thm:DP-agnostic}, we may show that
\begin{equation}
\label{eq:agnostic-jump1}
\sum_{I \in \mathcal{J}_1} \sum_{i \in I} (f (\vec{x}_i) - \fhat (\vec{x}_i))^2 \leq \sigma^2 \left( k + O \left( \log \frac{n}{\delta} \right) \sqrt{m} \right) + O \left(k \sigma \log \frac{n}{\delta} \left( n \cdot \OPT_k \right)^{1/2} \right) + n \cdot \OPT \; .
\end{equation}
Finally, we bound the error on $\mathcal{J}_2$.
Fix an $I \in \mathcal{J}_2$, and let $M_1, \ldots, M_{k / \tau}$ be as before.
Recall that this proof had two components: an upper bound for the $M_1, \ldots, M_\ell$ and a lower bound for $I$.
We first compute the upper bound, by following the calculations for Equation \ref{eq:upper-bound} and using Lemma \ref{lem:agnostic-flat} we have
\begin{align*}
\sum_{i = 1}^{k / \tau} \left( \sum_{i \in M_\ell} (y_i - \fLS^{M_\ell} (\vec{x}_i) )^2 - s^2 |M_\ell| \right) &\leq O \left( \frac{k}{\tau} \sigma^2 \left(r+ \log \left( \frac{n}{\delta} \right) \right) + \sigma \log\left( \frac{n}{\delta} \right)\sqrt{n} \right. \\
&\left. + \frac{k}{\tau} \sigma \log \left( \frac{n}{\delta} \right) \left( n \cdot \OPT_k \right)^{1/2} + n \cdot \OPT_k \right)
\end{align*}
The lower bound is in fact unchanged: we may use Equation \ref{eq:lower-bound} as stated.
Putting these two terms together and simplifying as we did previously, we obtain that
\begin{align*}
\sum_{i \in I} (f(\vec{x}_i) - \fhat(\vec{x}_i))^2 &\leq O \left( \sigma^2 \left(r + \log \left( \frac{n}{\delta} \right) \right) + \sigma \log \frac{n}{\delta} \left( \frac{\tau \sqrt{n}}{k}  + \sqrt{|I|} \right) \right.\\
&\left.+ \sigma \log \left( \frac{n}{\delta} \right) \left( n \cdot \OPT_k \right)^{1/2} + \frac{\tau}{k} n \cdot \OPT_k \right) \; .
\end{align*}
Summing up all the bounds we have achieved as we did previously demonstrates the desired claim.
\end{proof}

Through virtually identical methods we also obtain the same upper bound for \textsc{BucketGreedyMerge} and \textsc{PostprocessedBucketGreedyMerge}.
We state the results but omit their proofs for this reason.

\begin{theorem}
Let $\fhat$ be the $m$-piecewise linear function that is returned by \textsc{BucketGreedyMerge}, where $m = (2 + \frac{2}{\tau}) k \log n + \gamma$.
Then, with probability $1 - \delta$, we have
\[\MSE (\fhat) \leq O\left( \sigma^2 \left( \frac{m( r +  \log (n / \delta) ) }{n} \right) + \sigma \sqrt{\frac{k}{n}} \log \left( \frac{n}{\delta} \right) + k \sigma \log \left( \frac{n}{\delta} \right) \sqrt{\frac{\OPT_k }{n}} + \tau \cdot \OPT_k \right) \; .\]
\end{theorem}

\begin{theorem}
Fix $\delta > 0$.
Let $\fhat_p$ be the estimator output by \textsc{PostprocessedBucketGreedyMerge}.
Then, with probability $1 - \delta$, we have
\[
\MSE (\fhat_p) \leq O \left( \frac{k \sigma^2 \left( r + \log \frac{n}{\delta} \right)}{n} + \sigma  \log \left( \frac{n}{\delta} \right) \sqrt{\frac{k}{n}} + k \sigma \log \left( \frac{n}{\delta} \right) \sqrt{\frac{\OPT_k }{n}} + \tau \cdot \OPT_k\right)
 \; .\]
\end{theorem}


==> binning.tex <==
\section{The binning algorithm}
\label{sec:binning}

The algorithm described above requires us to exactly what $\sigma^2$ is, or at least have a pretty good guess.
In practice, ?????????

In this section we give a variant of the above algorithm which does not require the algorithm to know $\sigma^2$.
At a high level, TODO.
The formal algorithm is given in Algorithm TODO.

\subsection{Analysis of \textsc{BucketGreedyMerge}}
This section is dedicated to the proof of the following theorem:
\begin{theorem}
\label{thm:bucket}
Let $\fhat$ be the $O(k \log n)$ histogram that is returned by \textsc{BucketGreedyMerge}.
Then, with probability $1 - \delta$, we have
\[\MSE (\fhat) \leq ??? \; .\]
\end{theorem}
\begin{proof}
As in the proof of Theorem \ref{thm:greedy}, we let $\mathcal{I}$ be the final partition of $[n]$ that our algorithm produces.
We again partition $\setI$ into two sets $\mathcal{F}$ and $\mathcal{J}$ as before, and further subdivide $\mathcal{J}$ into $\mathcal{J}_1$ and $\mathcal{J}_2$.
The error on $\mathcal{F}$ and $\mathcal{J}_1$ is the same as the error given in Equations \ref{eq:flat} and \ref{eq:jump1}.
The only difference is the error on intervals in $\mathcal{J}_2$.

Let $I \in \mathcal{J}_2$ be fixed.
By definition this means there was some iteration and a collection of some $k + 1$ disjoint intervals $M_1, \ldots, M_{k + 1}$ so that $|M_\ell| / 2 \leq |I| \leq 2 |M_\ell|$ and
\[\frac{1}{|I|} \sum_{i \in I} (y_i - \fhat(\vec{x}_i))^2 \leq \frac{1}{|M_\ell|} \sum_{i \in M_\ell} (y_i - \fLS^{M_\ell} (\vec{x}_i))^2\]
for all $\ell = 1, \ldots, k + 1$.
Since $f$ has at most $k$ discontinuities, this means that there is at least one $M_\ell$ so that $f$ is continuous on $M_\ell$.
WLOG assume that $f$ is continuous on $M_1$.
By the same kinds of calculations done in the proof of Theorem \ref{thm:greedy}, we have that with probability $1 - \delta$,
\[\sum_{i \in M_1} (y_i - \fLS^{M_\ell} (\vec{x}_i))^2 \leq  O \left( \sigma^2 ( R + \log (1 / \delta) ) \right) + \sigma^2 \left( |M_\ell| + O(\log n / \delta) \sqrt{|M_\ell|} \right)\]
and
\[\sum_{i \in I} (y_i - \fhat (\vec{x}_i))^2 \geq  \sum_{i \in I} (f(\vec{x}_i) - \fhat (\vec{x}_i))^2 -  O \left( \sigma^2 (R + \log (1 / \delta) ) \right) + \sigma^2 \left( |I| - O(\log n / \delta) \sqrt{|I|} \right) \]
and putting these two equations together and rearranging, we have
\begin{align*}
\sum_{i \in I} (f(\vec{x}_i) - \fhat (\vec{x}_i))^2 &\leq O \left( \sigma^2 (R + \log (1 / \delta) ) \right) + \sigma^2 \cdot O(\log n / \delta) \left( \frac{|I|}{\sqrt{|M_\ell|}} + \sqrt{|I|} \right) \\
&\leq  O \left( \sigma^2 (R + \log (1 / \delta) ) \right) + O\left( \sigma^2 \log (n / \delta) \sqrt{|I|} \right) \; ,
\end{align*}
where the last inequality used that $|M_\ell| \geq |I| / 2$.
Since there are at most $k$ elements in $\mathcal{J}_2$, and they are all disjoint, this yields that
\begin{equation}
\label{eq:bucketjump}
\sum_{I \in \mathcal{J}_2} \sum_{i \in I} (f(\vec{x}_i) - \fhat (\vec{x}_i))^2 \leq O \left( k \sigma^2 (R + \log (1 / \delta) ) \right) + O\left( \sigma^2 \log (n / \delta) \sqrt{k n} \right)
\end{equation}
and putting this equation together with Equations \ref{eq:flat} and \ref{eq:jump1} yields the desired conclusion.
\end{proof}


==> contributions.tex <==
\section{Our contributions}
\label{sec:contributions}

In this paper, we study the problem of fixed design segmented regression.
We are given samples $\vec{x}_i \in \R^d$, for $i = 1, \ldots, n$, and we consider the following classical regression model:
\begin{equation}
\label{eq:model}
y_i = f(\vec{x}_i) + \epsilon_i \; .
\end{equation}
Here, the $\epsilon_i$ are independent sub-Gaussian noise variables with variance proxy $\sigma^2$ and $\EE [\epsilon_i] = 0$ for all $i$,
and we will assume that $f: \R^d \to \R$ is a $t$-piecewise linear function, or well-approximated by one.
Formally, we mean:
\begin{definition}
Let $f: \R^d \to \R$.
We say that $f$ is a \emph{$k$-piecewise linear} function if there exists a partition of the real line into $t$ disjoint intervals $I_1, \ldots, I_k$ and $t$ corresponding parameters $\vec{\theta}_1, \ldots, \vec{\theta}_k \in \R^d$ so that for all $\vec{x} = (x_1, \ldots, x_d) \in \R^d$, we have that $f(x) = \langle \vec{\theta}_i, x \rangle$ if $x_1 \in I_i$.
Let $\mathcal{L}_k$ denote the space of $k$-piecewise linear functions.

Moreover, we say $f$ is continuous on an interval $I \subseteq \R$ if $I \subseteq I_i$ for some $i = 1, \ldots, t$, otherwise, we say that $f$ is discontinuous on $I$.
\end{definition}

Following this generative model, the algorithm is given the $n$ pairs $(\vec{x_i}, y_i)$ as input.
The goal of the algorithm is to produce an estimate $\fhat$ that is close to the true, unknown $f$ with high probability over the noise terms $\epsilon_i$ and any randomness in the algorithm.
Here and throughout the paper, we use the classical mean-squared error:
\[\MSE (\fhat) = \frac{1}{n} \sum_{i = 1}^n (f(\vec{x_i}) - \fhat(\vec{x_i}))^2 \; .\]

We remark that this model as contains the problem of (fixed design) piecewise polynomial regression as an important subcase. \todo{say more here}

We also consider the agnostic model. \todo{say more here}

\subsection{Mathematical Preliminaries}
In this section we state some preliminaries that our analysis builds on.

\paragraph{Tail bounds.}
We will require the following tail bound on sub-exponential random variables:
\begin{theorem}[Bernstein-type inequality c.f. ????]
\label{thm:bernstein}
Let $X_1, \ldots, X_N$ be centered sub-exponential random variables, and let $K = \max_i \| X_i \|_{\phi_1}$.
Then for all $t > 0,$ and for $N \geq t^2 / K^2$, we have
\[\Pr \left[ \left| \frac{1}{\sqrt{N}} \sum_{i = 1}^N X_i \right| \geq t \right] \leq 2 \exp \left[ -c \frac{t^2}{K^2} \right] \; .\]
\end{theorem}
Since the regime we are interested in will have $N$ to be much larger than $t$, for the rest of the paper we will assume that the condition that $N \geq t^2 / K^2$ holds.
\paragraph{Linear regression}
Our analysis builds on the classical results for fixed design linear regression.
In linear regression, the generative model is exactly of the form described in Equation \ref{eq:model}, except $f$ is now a linear function (instead of a piecewise linear function), i.e., $f(\vec{x}) = \langle \theta^\ast, \vec{x} \rangle$ for some unknown $\theta^\ast$.
This problem is very well understood, and the asymptotically best estimator is known to be the \emph{least-squares} estimator.
\begin{definition}
Given $\vec{x}_1, \ldots, \vec{x}_n$ and $y_1, \ldots, y_n$, the \emph{least squares estimator} $\fLS$ is defined to be the linear function which minimizes $\sum_{i = 1}^n (y_i - f(\vec{x}_i))^2$ over all linear functions $f$.
For an interval $I \subseteq \{1, \ldots, n\}$, we let $\fLS^I$ be the least-squares estimator for the data $\{(\vec{x}_i, y_i) \}_{i \in I}$.
\end{definition}
For the least-squares estimator, the following prediction error rate is known:
\begin{theorem}
\label{thm:LSrate}
Let $\vec{x}_1, \ldots, \vec{x}_n$ and $y_1, \ldots, y_n$ be generated as Equation \ref{eq:model}, where $f$ is a linear function. Let $\fLS (x)$ be the least squares estimator. Let $\vec{X} \in \R^{n \times d}$ be the matrix whose $j$th row is $\vec{x}_j^T$. Then,
\[\EE \left[ \MSE (\fLS) \right] = O \left( \sigma^2 \frac{r}{n} \right) \; ,\]
where $r = \rank (\vec{X}^T \vec{X})$.
Moreover, with probability $1 - \delta$, we have
\[\MSE (\fLS) = O\left( \sigma^2 \frac{r + \log 1 / \delta}{n} \right) \; . \]
\end{theorem}

Theorem \ref{thm:LSrate} can be proved with the following lemma, which we will also require.
The lemma bounds the correlation of a random vector with any fixed r-dimensional subspace:
\begin{lemma}
\label{lem:incoherence}
Fix $\delta > 0$.
Let $\epsilon_1, \ldots, \epsilon_n$ be i.i.d. sub-gaussian random variables with variance proxy $\sigma^2$.
Let $\vec{\epsilon} = (\epsilon_1, \ldots, \epsilon_n)$, and let $S$ be a fixed $r$-dimensional affine subspace of $\R^n$.
Then, with probability $1 - \delta$, we have
\[\sup_{\vec{v} \in S} \frac{| \vec{v}^T \vec{\epsilon} |}{\| \vec{v} \|} \leq O(\sigma \sqrt{r + \log 1 / \delta}) \; . \]
\end{lemma}

This lemma yields the following straightforward consequence:
\begin{corollary}
\label{cor:sim-incoherence}
Fix $\delta > 0$.
Let $\epsilon_1, \ldots, \epsilon_n$ be as in Lemma \ref{lem:incoherence}.
Then with probability at least $1 - \delta$, we have
\[\sup_{f \in \mathcal{L}_k} \frac{\left| \sum_{i = 1}^n \epsilon_i f(\vec{x}_i) \right|}{\left( \sum_{i = 1}^n f(\vec{x}_i) \right)^2} \leq O \left( \sigma \sqrt{k r + k \log \frac{n}{\delta}} \right) \; . \]
\end{corollary}
\begin{proof}
Fix any partition of $[n]$ into $k$ intervals $\setI$, and let $S_\setI$ be the set of $k$-piecewise linear functions which are continuous on each $I \in \setI$.
Then it is not hard to see that $S_\setI$ is a $kr$ dimensional linear subspace, and hence, by Lemma \ref{lem:incoherence}, we have that 
\[\sup_{f \in S_\setI} \frac{\left| \sum_{i = 1}^n \epsilon_i f(\vec{x}_i) \right|}{\left( \sum_{i = 1}^n f(\vec{x}_i) \right)^2} \leq O \left( \sigma \sqrt{k r + \log \frac{1}{\delta'}} \right)\]
with probability at least $1 - \delta'$.
By a basic stars-and-bars argument is is not hard to see that there are $\binom{n - k}{k} = n^{O(k)}$ such different partitions $\setI$.
Let $\delta' = \delta / \binom{n - k}{k}$.
Then the result follows by union bounding over all the different possible partitions.
\end{proof}
\todo{Figure out runtimes for finding least squares, see CW13 among others}

\subsection{Background}

\subsection{Notation (TEMPORARY)}
\begin{itemize}
\item $f$ is truth, $\fLS$ is least squares fit
\item data points $\vec{x}_1, \ldots, \vec{x}_n$
\item noise $\epsilon_1, \ldots, \epsilon_n$ with variance proxy $\sigma^2$
\item responses are $y_1, \ldots, y_n$
\item for intervals $I$, $f^I$, $\fLS^I$, $\fhat^I$ etc all mean the restriction to $I$. In particular, $\fLS^I$ is the least squares fit on $I$.
\item Similarly $\vec{x}^I$ and $y^I$ as above.
\item $\MSE$ is mean-squared error
\item $R$ is the maximum rank of any submatrix of the data matrix.
\end{itemize}

\subsection{Analysis of the exact DP}
\begin{theorem}
\label{thm:DP}
Let $\delta > 0$, and let $\fLS$ be the $k$-piece linear estimator returned by the exact DP.
Then, with probability $1 - \delta$, we we have that
\[\MSE (\fLS) \leq O(???) \; .\]
\end{theorem}
\begin{proof}
We follow the proof technique for convergence of linear least squares as presented in RIG-NOTES \todo{find right citation}.
Recall $f$ is the true $k$-piece linear estimator.
Then, by the definition of the least squares fit, we have that
\begin{align*}
\sum_{i = 1}^n (y_i - \fLS(\vec{x}_i))^2 &\leq \sum_{i = 1}^n (y_i - f(\vec{x}_i))^2 \\
&= \sum_{i = 1}^n \epsilon_i^2 \; .
\end{align*}
By expanding out the LHS, we have that
\begin{align*}
\sum_{i = 1}^n (y_i - \fLS(\vec{x}_i))^2 &= \sum_{i = 1}^n ( f(\vec{x}_i) + \epsilon_i - \fLS(\vec{x}_i))^2 \\
&= \sum_{i = 1}^n (\fLS (\vec{x}_i) - f(\vec{x}_i))^2 + 2 \sum_{i = 1}^n \epsilon_i (\fLS (\vec{x}_i) - f(\vec{x}_i)) + \sum_{i = 1}^n \epsilon_i^2 \ .
\end{align*}
From these two calculations we gather that
\begin{align*}
\sum_{i = 1}^n (\fLS (\vec{x}_i) - f(\vec{x}_i))^2 &\leq 2 \sum_{i = 1}^n \epsilon_i (\fLS (\vec{x}_i) - f(\vec{x}_i)) \\
&\leq 2 \sup_{\mbox{$g \in \mathcal{L}_k$}}\sum_{i = 1}^n \epsilon_i (g (\vec{x}_i) - f(\vec{x}_i)) \\
&\leq O \left( \sigma \sqrt{kr + k \log \frac{n}{\delta}} \right) \cdot \left( \sum_{i = 1}^n (\fLS (\vec{x}_i) - f(\vec{x}_i))^2 \right)^{1/2} \; ,
\end{align*}
with probability $1 - \delta$, where the last line follows from Corollary \ref{cor:sim-incoherence}.
A simple algebraic manipulation  from this last inequality yields the desired statement.
\end{proof}

The same proof can also be easily adapted to show the following extension of Theorem \ref{thm:LSrate}:
\begin{lemma}
\label{lem:flat}
Fix $\delta > 0$.
Then with probability $1 - \delta$,
\[\sum_{\ell = 1}^k \sum_{i \in J_\ell} (g(\vec{x}_i) - f(\vec{x}_i))^2 \leq O (\sigma^2 k (r + \log (n / \delta))) \; ,\]
simultaneously, for all disjoint sets of $k$ intervals $J_1, \ldots, J_k$ of $[n]$, where on each $J_\ell$, the function $g$ is the least squares fit to the data on $J_\ell$.
\end{lemma}


==> latexdefs.tex <==
\declaretheorem{theorem}
\declaretheorem[sibling=theorem]{definition}
\declaretheorem[sibling=theorem]{lemma}
\declaretheorem[sibling=theorem]{corollary}
\declaretheorem[sibling=theorem]{fact}
\declaretheorem{example}
\declaretheorem[numbered=no]{problem}

\newcommand{\new}[1]{{\color{red} #1}}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}

\newcommand{\eps}{\ensuremath{\epsilon}}
\newcommand{\fhat}{\ensuremath{\widehat{f}}}
\newcommand{\setI}{\mathcal{I}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\polylog}{\mathrm{polylog}}
\newcommand{\Otilde}{\ensuremath{\widetilde{O}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\that}{\ensuremath{\widehat{\vec{\theta}}}}
\newcommand{\MSE}{\ensuremath{\mathrm{MSE}}}
\newcommand{\LS}{{\mathrm{LS}}}
\newcommand{\thatLS}{\that_{\LS}}
\newcommand{\fLS}{\ensuremath{{f_{\LS}}}}
\renewcommand{\vec}[1]{\ensuremath{\bm{#1}}}
\newcommand{\rank}{\ensuremath{\mathrm{rank}}}
\newcommand{\OPT}{\ensuremath{\mathrm{OPT}}}
\newcommand{\ve}[1]{\ensuremath{\bm{#1}}}


==> merging.tex <==
\section{A greedy merging algorithm}
\label{sec:merging}
In this section, we formally state our new algorithm for segmented regression and analyze its statistical and computational efficiency.
See Algorithm \ref{alg:greedy} for the corresponding pseudocode.
The algorithm expects two tuning parameters $\tau, \gamma$ because the algorithm does not return a $k$-piecewise linear function but instead a $O(k)$-piecewise linear function
The tuning parameters allow us to trade off running time for fewer pieces.
In typical use cases we have $\tau, \gamma = \Theta(1)$, in which case our algorithm produces an $O(k)$-piecewise linear function in time $O(n d^2 \log n)$ time.

\begin{algorithm*}[htb]
\begin{algorithmic}[1]
\STATE $\textsc{GreedyMerging}(\tau, \gamma, s, \vec{X}, \vec{y})$

\COMMENT{\emph{Initial partition of $[n]$ into intervals of length $1$.}}
\STATE $\setI^0 \gets \{\{ 1 \}, \{ 2 \}, \ldots, \{ n \}\}$ 
%\vspace{.2cm}

\COMMENT{\emph{Iterative greedy merging (we start with $j \gets 0$).}}
%\State $j \gets 0$
\WHILE{$| \setI^j | > (2 + \frac{2}{\tau}) k + \gamma$}
  \STATE Let $s_j$ be the current number of intervals.
  %\vspace{.2cm}
  \COMMENT{\emph{Compute the least squares fit and its error for merging neighboring pairs of intervals.}}
  \FOR{$u \in \{1, 2, \ldots, \frac{s_j}{2}\}$}
    \STATE $\theta_u \gets \textsc{LeastSquares}(\vec{X}, \vec{y}, I_{2u - 1} \cup I_{2u})$
    \STATE $e_u = \| \vec{y}^I - \vec{X}^I \theta_u \|_2^2 - s^2 |I_{2u - 1} \cup I_{2u}|$
  \ENDFOR
  \STATE Let $L$ be the set of indices $u$ with the $(1 + \frac{1}{\tau})k$ largest errors $e_u$, breaking ties arbitrarily.
  \STATE Let $M$ be the set of the remaining indices. 
  %\vspace{.2cm}
  %\LineComment{Keep the intervals with the large merging errors.}
  \COMMENT{\emph{Keep the intervals with large merging errors.}}
  \STATE $\setI^{j+1} \gets \bigcup\limits_{u \in L} \{I_{2u - 1}, I_{2u}\}$ 
  %\LineComment{Merge the remaining intervals.}
  \COMMENT{\emph{Merge the remaining intervals.}}
  \STATE $\setI^{j+1} \gets \setI^{j+1} \cup \{I_{2u - 1} \cup I_{2u} \, | \, u \in M \}$ 
  %\vspace{.2cm}
  \STATE $j \gets j + 1$
\ENDWHILE
%\vspace{.2cm}
\STATE \textbf{return} the least squares fit to the data on every interval in $\setI^j$
\end{algorithmic}
\caption{Piecewise linear regression by greedy merging.}
\label{alg:greedy}
\end{algorithm*}

We now state the running time of \textsc{GreedyMerging}.
The analysis is similar to the analysis presented in \cite{ADHLS15} and for space considerations is left to the supplementary material.
\begin{theorem}
\label{thm:time-greedy}
Let $\vec{X}$ and $\vec{y}$ be as above. Then $\textsc{GreedyMerging}(\tau, \gamma, s, \vec{X}, \vec{y})$ outputs a $\left( (2 + \frac{2}{\tau}) k + \gamma \right)$-piecewise linear function and runs in time $O(nd^2 \log(n / \gamma))$.
\end{theorem}

\subsection{Analysis of \textsc{GreedyMerging}}


\begin{theorem}
\label{thm:greedy}
Let $\delta > 0$, and let $\fhat$ be the estimator returned by \textsc{GreedyMerging}.
Let $m = (2 + \frac{2}{\tau}) k + \gamma$ be the number of pieces in $\fhat$.
Then, with probability $1 - \delta$, we have that
\begin{align*}
&\MSE (\fhat)  \\
 &\; \leq O\left( \sigma^2 \left( \frac{m (r + \log (n / \delta) )}{n} \right) + \sigma \frac{\tau + \sqrt{k}}{\sqrt{n}} \log \left( \frac{n}{\delta} \right) \right) \, .
\end{align*}
\end{theorem}


\begin{proof}
We first condition on the event that Corollaries \ref{cor:unif-err-bound}, \ref{cor:int-incoherence} and \ref{cor:sim-incoherence}, and Lemma \ref{lem:flat} all hold with error parameter $O(\delta)$, so that together they all hold with probability at least $1 - \delta$.
Let $\setI = \{ I_1, \ldots, I_{m} \}$ be the final partition of $[n]$ that our algorithm produces.
Recall $f$ is the ground truth $k$-piecewise linear function.
We partition the intervals in $\setI$ into two sets:  
\begin{align*}
\mathcal{F} &= \{I \in \setI: \mbox{$f$ is flat on $I$} \} \; ,\\
\mathcal{J} &= \{I \in \setI: \mbox{$f$ has a jump on $I$} \} \; .
\end{align*}
We first bound the error over the intervals in $\mathcal{F}$.
By Lemma \ref{lem:flat}, we have
\begin{equation}
\label{eq:flat}
\sum_{I \in \mathcal{F}} \norm{\vec{f}_I - \vec{\fhat}_I}^2 \; \leq \; O (\sigma^2 |\mathcal{F}| (r + \log ( n / \delta))) \;,
\end{equation}
with probability at least $1 - O(\delta)$.

We now turn our attention to the intervals in $\mathcal{J}$ and distinguish two further cases.
We let $\mathcal{J}_1$ be the set of intervals in $\mathcal{J}$ which were never merged, and we let $\mathcal{J}_2$ be the remaining intervals.
If the interval $I \in \mathcal{J}_1$ was never merged, the interval contains one point, call it $i$.
Because we may assume that $\vec{x}_i \neq 0$, we know that for this one point, our estimator satisfies $\fhat (\vec{x}_i) = y_i$, since this is clearly the least squares fit for a linear estimator on one nonzero point.
Hence Corollary \ref{cor:unif-err-bound} implies that the following inequality holds with probability at least $1 - O(\delta)$:
\begin{align*}
\sum_{I \in \mathcal{J}_1} \norm{\vec{f}_I - \vec{\fhat}_I}^2 &= \sum_{I \in \mathcal{J}_1} \norm{\epsilon_I}^2 \\
&\leq \sigma^2 \left( \sum_{I \in \mathcal{J}_1} |I| + O \left( \log \frac{n}{\delta} \right) \sqrt{\sum_{I \in \mathcal{J}_1} |I|} \right) \\
&\leq \sigma^2 \left( m + O \left( \log \frac{n}{\delta} \right) \sqrt{m} \right) \; . \numberthis \label{eq:jump1}
\end{align*}

We now finally turn our attention to the intervals in $\mathcal{J}_2$.
Fix an interval $I \in \mathcal{J}_2$.
By definition, the interval $I$ was merged in some iteration of the algorithm.
This implies that in that iteration, there were $(1 + 1 / \tau) k$ intervals $M_1, \ldots, M_{(1 + 1/ \tau) k}$ so that for each interval $M_\ell$, we have
\begin{equation}
\label{eq:merge-cond}
\norm{\vec{y}_I - \vec{\fhat}_I}^2 - s^2 |I| \; \leq \; \norm{\vec{y}_{M_\ell} - \vecfLS_{M_\ell}}^2 - s^2 |M_\ell| \; .
\end{equation}
Since the true, underlying $k$-piecewise linear function $f$ has at most $k$ jumps, this means that there are at least $k / \tau$ intervals of the $M_\ell$ on which $f$ is flat.
WLOG assume that these intervals are $M_1, \ldots, M_{k / \tau}$.

We have, by definition,
\begin{align*}
&\sum_{\ell = 1}^{k / \tau} \left\| \vec{y}_{M_\ell} - \vecfLS_{M_\ell} \right\|^2 - s^2 |M_\ell|  =  \sum_{\ell = 1}^{k / \tau} \left\| \vec{f}_{M_\ell} - \vecfLS_{M_\ell} \right\|^2 \\
& + 2 \sum_{\ell = 1}^{k / \tau} \langle \vec{\epsilon}_{M_\ell}, \vec{f}_{M_\ell} - \vecfLS_{M_\ell} \rangle + \sum_{\ell = 1}^{k / \tau}\sum_{i \in M_\ell} (\epsilon_i^2 - s^2) \; . \numberthis \label{eq:flat-allterms}
\end{align*}
We will upper bound each term on the RHS in turn.
First, since the function $f$ is flat on each $M_\ell$ for $\ell = 1, \ldots, k / \tau$, Lemma \ref{lem:flat} implies
\begin{equation}
\label{eq:flat-term1}
\sum_{\ell = 1}^{k / \tau} \left\| \vec{f}_{M_\ell} - \vecfLS_{M_\ell} \right\|^2 \leq O \left(\sigma^2 \frac{k}{\tau} \left(r + \log \frac{n}{\delta} \right) \right) \; , \end{equation}
with probability at least $1 - O(\delta)$.

Moreover, note that the function $\fls_{M_\ell}$ is a linear function on $M_\ell$ of the form $\fls_{M_\ell}(\vec{x}) = \vec{x}^T \hat{\beta}$, where $\hat{\beta} \in \R^d$ is the least-squares fit on $M_{\ell}$.
Because $\vec{f}$ is just a fixed vector, the vector $\vec{f}_{M_\ell} -\vecfLS_{M_\ell} $ lives in the affine subspace of vectors of the form $\vec{f}_{M_\ell} + (\vec{X}_{M_\ell}) \eta$ where $\eta \in \R^d$ is arbitrary.
So Corollary \ref{cor:sim-incoherence} and~\eqref{eq:flat-term1} imply that
\begin{align*}
&\sum_{\ell = 1}^{k / \tau}\langle \vec{\epsilon}_{M_\ell}, \vec{f}_{M_\ell} - \vecfLS_{M_\ell} \rangle \\
&\leq \sqrt{\sum_{\ell = 1}^{k / \tau}\langle \vec{\epsilon}_{M_\ell}, \vec{f}_{M_\ell} - \vecfLS_{M_\ell} \rangle} \cdot \sup_{\eta} \frac{|\langle \vec{\epsilon}_{M_\ell},  \vec{X} \eta \rangle |}{\| \vec{X} \eta \|} \\
&\leq O \left(\sigma^2 \frac{k}{\tau} \left(r + \log \frac{n}{ \delta} \right) \right)\; . \numberthis \label{eq:flat-term2}
\end{align*}
with probability $1 - O(\delta)$.

By Corollary \ref{cor:unif-err-bound}, we get that with probability $1 - O(\delta)$,
\[\sum_{\ell = 1}^{k / \tau} \left( \sum_{i \in M_\ell} \epsilon_i^2 - s^2 |M_\ell| \right) \leq O\left( \sigma \log \frac{n}{\delta} \right) \sqrt{n} \; .\]
Putting it all together, we get that
\begin{align*}
&\sum_{i = 1}^{k / \tau} \left( \left\| \vec{y}_{M_\ell} - \vecfLS_{M_\ell} \right\|^2 - s^2 |M_\ell|  \right) \\
&\leq O \left(\frac{k}{\tau} \sigma^2 \left(r+ \log \frac{n}{\delta} \right) \right) + O\left(\sigma \log \frac{n}{\delta} \right) \sqrt{n} \;  \numberthis \label{eq:flat-term3} 
\end{align*}
with probability $1 - O(\delta)$.
Since the LHS of~\eqref{eq:merge-cond} is bounded by each individual summand above, this implies that the LHS is also bounded by their average, which implies that
\begin{align*}
&\norm{\vec{y}_I - \vec{\fhat}_I}^2 - s^2 |I| \\ 
&\leq \frac{\tau}{k} \sum_{i = 1}^{k / \tau} \left( \norm{\vec{y}_{M_\ell} - \vecfls_{M_\ell}}^2 - s^2 |M_\ell| \right) \\
&\leq  \; O\left(\sigma^2 \left(r + \log \left( \frac{n}{\delta} \right) \right) \right) + O\left(\sigma \log \frac{n}{\delta} \right) \frac{\tau \sqrt{n}}{k} \; . \numberthis \label{eq:upper-bound}
\end{align*}
We now similarly expand out the LHS of~\eqref{eq:merge-cond}:
\begin{align*}
&\norm{\vec{y}_I - \vec{\fhat}_I}^2 - s^2 |I| \\
&= \norm{\vec{f}_I + \vec{\epsilon}_I - \vec{\fhat}_I}^2 - s^2 |I| \\
&= \norm{\vec{f}_I - \vec{\fhat}_I}^2 + 2 \langle \vec{\epsilon}_I, \vec{f}_I - \vec{\fhat}_I \rangle + \norm{\vec{\epsilon}_I}^2 - s^2 |I|  \; . \numberthis \label{eq:jump-allterms}
\end{align*}
Next, we aim to upper bound $\sum_{i \in I} (f (\vec{x}_i) - \fhat (\vec{x}_i))^2$.
Hence, we lower bound the second and third terms of~\eqref{eq:jump-allterms}.
The calculations here closely mirror those above.

By Corollary \ref{cor:int-incoherence}, we have that
\[ 
2 \langle \vec{\epsilon}_I, \vec{f}_I - \vec{\fhat}_I \rangle \; \geq \; - O \left(\sigma \sqrt{r + \log \left( \frac{n}{\delta} \right)} \right) \norm{\vec{f}_I - \vec{\fhat}_I} \; ,
\]
and by Corollary \ref{cor:unif-err-bound} we have
\[
\norm{\vec{\epsilon}_I}^2 - s^2 |I| \; \geq \; - O \left(\sigma \log \frac{n}{\delta} \right) \sqrt{|I|} \; ,
\]
and so
\begin{align*}
&\norm{\vec{y}_I - \vec{\fhat}_I}^2 - s^2 |I| \\
&\geq \norm{\vec{f}_I - \vec{\fhat}_I}^2 - O \left(\sigma \sqrt{r + \log \left( \frac{n}{\delta} \right)} \right) \norm{\vec{f}_I - \vec{\fhat}_I} \\
&~~~~~- O\left(\sigma \log \frac{n}{\delta} \right) \sqrt{|I|} \; . \numberthis \label{eq:lower-bound}
\end{align*}
Putting~\eqref{eq:upper-bound} and~\eqref{eq:lower-bound} together yields that with probability $1 - O(\delta)$,
\begin{align*}
\norm{\vec{f}_I - \vec{\fhat}_I}^2 \; &\leq \; O\left( \sigma^2 \left(r + \log \left( \frac{n}{\delta} \right) \right) \right) \\
&~~~~~+ O \left(\sigma \sqrt{r + \log \left( \frac{n}{\delta} \right)} \right) \norm{\vec{f}_I - \vec{\fhat}_I}  \\
&~~~~~+ O\left( \sigma \log \frac{n}{\delta} \right) \left( \frac{\tau \sqrt{n}}{k} + \sqrt{|I|} \right) \; .
\end{align*}

Letting $z^2 = \norm{\vec{\fhat}_I - \vec{f}_I}^2$, then this inequality is of the form $z^2 \leq b z + c$ where $b, c \geq 0$.
In this case, we have that
\begin{align*}
b &= O \left( \sigma \sqrt{r + \log \frac{n}{\delta} } \right) \; ,~ \mbox{and} \\
c &= O \left( \sigma^2 \left(r + \log \left( \frac{n}{\delta} \right) \right) \right) + O\left( \sigma \log \frac{n}{\delta} \right) \left( \frac{\tau \sqrt{n}}{k} + \sqrt{|I|} \right)
\end{align*}
We now prove the following lemma about the behavior of such quadratic inequalities:
\begin{lemma}
\label{lem:quadratic}
Suppose \newjd{$z^2 \leq bz + c$} where $b, c \geq 0$.
Then $z^2 \leq O(b^2 + c)$.
\end{lemma}
\begin{proof}
From the quadratic formula, the inequality implies that \newjd{$z \leq \frac{b + \sqrt{b^2 + 4c}}{2}$}.
From this, it is straightforward to demonstrate the desired claim.
\end{proof}
Thus, from the lemma, we have
\begin{align*}
&\norm{\vec{f}_I - \vec{\fhat}_I}^2 \; \leq \; O\left( \sigma^2 \left(r + \log \left( \frac{n}{\delta} \right) \right) \right) \\
 &~~~~~+ O\left( \sigma \log \frac{n}{\delta} \right) \left( \frac{\tau \sqrt{n}}{k} + \sqrt{|I|} \right) \; .
\end{align*}

Hence the total error over all intervals in $\mathcal{J}_2$ can be bounded by:
\begin{align*}
&\sum_{I \in \mathcal{J}_2} \norm{\vec{f}_I - \vec{\fhat}_I}^2 \;  \leq \; O \left(k \sigma^2 \left(r + \log \left( \frac{n}{\delta} \right) \right) \right) \\
&~~~~~~+ O\left( \sigma \log \frac{n}{\delta} \right) \left( \tau \sqrt{n} + \sum_{I \in \mathcal{J}}\sqrt{|I|} \right) \\
&\; \leq O \left( k \sigma^2 \left(r + \log \left( \frac{n}{\delta'} \right) \right) \right) \\
&~~~~~~+ O\left(\sigma \log \frac{n}{\delta} \right) \left( \tau \sqrt{n} + \sqrt{k n} \right) \numberthis \label{eq:jump2} \; .
\end{align*}
In the last line we use that the intervals $I \in \mathcal{J}_2$ are disjoint (and hence their cardinalities sum up to at most $n$), and that there are at most $k$ intervals in $\mathcal{J}_2$ because the function $f$ is $k$-piecewise linear.
Finally, applying a union bound and summing~\eqref{eq:flat},~\eqref{eq:jump1}, and~\eqref{eq:jump2} yields the desired conclusion.
\end{proof}




















==> prelims-icml.tex <==
\section{Preliminaries}
In this paper, we study the problem of fixed design segmented regression.
We are given samples $\vec{x}_i \in \R^d$ for $i \in [n] \, (\, = \{1,  \ldots, n\})$, and we consider the following classical regression model:
\begin{equation}
\label{eq:model}
y_i = f(\vec{x}_i) + \epsilon_i \; .
\end{equation}
Here, the $\epsilon_i$ are i.i.d.\ sub-Gaussian noise variables with variance proxy $\sigma^2$, mean $\EE [\epsilon_i] = 0$, and variance $s^2 = \EE[\epsilon_i^2]$ for all $i$. %\footnote{We observe that $s^2$ is guaranteed to be finite since the $\epsilon_i$ are sub-Gaussian. The variance $s^2$ is in general not equal to the variance proxy $\sigma^2$, however, it is well-known that $s^2 \leq \sigma^2$.}
We will let $\epsilon = (\epsilon_1, \ldots, \epsilon_n)$ denote the vector of noise variables.
We also assume that $f: \R^d \to \R$ is a $k$-piecewise linear function. 
Formally, this means:
\begin{definition}
The function $f: \R^d \to \R$ is a \emph{$k$-piecewise linear} function if there exists a partition of the real line into $k$ disjoint intervals $I_1, \ldots, I_k$, $k$ corresponding parameters $\vec{\theta}_1, \ldots, \vec{\theta}_k \in \R^d$, and a fixed, known $j$ such that for all $\vec{x} = (x_1, \ldots, x_d) \in \R^d$ we have that $f(\vec{x}) = \langle \vec{\theta}_i, \vec{x} \rangle$ if $x_j \in I_i$.
Let $\mathcal{L}_{k,j}$ denote the space of $k$-piecewise linear functions with partition defined on coordinate $j$.

Moreover, we say $f$ is \emph{flat} on an interval $I \subseteq \R$ if $I \subseteq I_i$ for some $i = 1, \ldots, k$, otherwise, we say that $f$ has a \emph{jump} on the interval $I$. \end{definition}

In the full paper, we also discuss the agnostic setting where the ground truth $f$ is not piecewise linear itself but only well-approximated by a $k$-piecewise linear function.
For simplicity of exposition, we assume that the partition coordinate $j$ is $1$ in the rest of the paper.
We remark that this model also contains the problem of (fixed design) piecewise polynomial regression as an important subcase (see the full paper for details).

Following this generative model, a regression algorithm receives the $n$ pairs $(\vec{x}_i, y_i)$ as input.
The goal of the algorithm is then to produce an estimate $\fhat$ that is close to the true, unknown $f$ with high probability over the noise terms $\epsilon_i$ and any randomness in the algorithm.
We measure the distance between our estimate $\fhat$ and the unknown function $f$ with the classical mean-squared error:
\[\MSE (\fhat) = \frac{1}{n} \sum_{i = 1}^n (f(\vec{x_i}) - \fhat(\vec{x_i}))^2 \; .\]

Throughout this paper, we let $\vec{X} \in \R^{n \times d}$ be the \emph{data matrix}, i.e., the matrix whose $j$-th row is $\vec{x}_j^T$ for every $j$, and we let $r$ denote the rank of $\vec{X}$. 
%We also assume that no $\vec{x}_i$ is the all-zeros vector, since such points are trivially fit by any linear function.

The following notation will also be useful.
For any function $f: \R^d \to \R$, we let $\vec{f} \in \R^{n}$ denote the vector with components $\vec{f}_i = f(\vec{x}_i)$ for \newjd{$i \in [n]$}.
 For any interval $I$, we let $\vec{X}^I$ denote the data matrix consisting of all data points $\vec{x}_i$ for $i \in I$, and for any vector $\vec{v} \in \R^n$, we let $\vec{v}^I \in \R^{|I|}$ be the vector of $\vec{v}_i$ for $i \in I$.

%Indeed, imagine we are given $x_1, \ldots, x_n \in \R$ and $y_1, \ldots, y_n \in \R$ so that there is some $k$-piece degree-$d$ polynomial $p$ so that for all $i = 1, \ldots, n$ we have $y_i = p(x_i) + \epsilon_i$, and our goal is to recover $p$ in the same mean-squared sense as above.
%We can write this problem as a $k$-piecewise linear fit in $\R^{d + 1}$, by associating the data vector $\vec{v}_i = (1, x_i, x_i^2, \ldots, x_i^{d})$ to each $x_i$.
%If the piecewise polynomial $p$ has breakpoints at $z_1, \ldots z_{k - 1}$, the associated partition for the $k$-piecewise linear function is $\setI = \{ (-\infty, z_1), [z_1, z_2), \ldots, (z_{k - 2}, z_{k - 1}], (z_{k-1}, \infty) \}$.
%If the piecewise polynomial is of the form $p(x) = \sum_{\ell = 0}^d a^I_\ell x^\ell$ for any interval $I \in \setI$, 
%then for any vector $\vec{v} = (v_1, v_2, \ldots, v_{d+1}) \in \R^{d + 1}$, the ground truth $k$-piecewise linear function is simply the linear function $f(\vec{v}) = \sum_{\ell = 1}^{d+1} a^I_{\ell-1} v_\ell$ for $v_2 \in I$.
%Moreover, the data matrix associated with the data points $\vec{v}$ is a Vandermonde matrix.
%For $n \geq d + 1$ it is well-known that this associated Vandermonde matrix has rank exactly $d + 1$ (assuming $x_i \neq x_j$ for any $i \neq j$).

\subsection{Our Contributions}
Our main contributions are new, fast algorithms for the aforementioned segmented regression problem.
We now informally state our main results and refer to later sections for more precise theorems.
\begin{theorem}[informal statement of Theorems \ref{thm:time-greedy} and \ref{thm:greedy}]
\label{thm:inf-greedy}
There is an algorithm \textsc{GreedyMerge}, which, given $\vec{X}$ (of rank $r$), $\vec{y}$, a target number of pieces $k$, and the variance of the noise $s^2$, runs in time $O(n d^2 \log n)$ and outputs an $O(k)$-piecewise linear function $\fhat$ so that with probability at least $0.99$, we have
\[
  \MSE (\fhat) \; \leq \; O\left(\sigma^2 \frac{kr}{n} + \sigma \sqrt{\frac{k}{n}} \log n \right) \; .
\]
\end{theorem}
That is, our algorithm runs in time which is \emph{nearly linear} in $n$ and still achieves a reasonable rate of convergence.
While this rate is asymptotically slower than the rate of the dynamic programming estimator, our algorithm is significantly faster than the DP so that in order to achieve a comparable MSE, our algorithm takes less total time given access to a sufficient number of samples.
For more details on this comparision and an experimental evaluation, see Sections \ref{sec:prior} and \ref{sec:experiments}.

At a high level, our algorithm first forms a fine partition of $[n]$ and then iteratively merges pieces of this partitions until only $O(k)$ pieces are left.
In each iteration, the algorithm reduces the number of pieces in the following manner: we group consecutive intervals into pairs which we call ``candidates''.
For each candidate interval, the algorithm computes an error term that is the error of a least squares fit combined with a regularizer depending on the variance of the noise $s^2$.
The algorithm then finds the $O(k)$ candidates with the largest errors.
We do not merge these candidates, but do merge all other candidate intervals.
We repeat this process until only $O(k)$ pieces are left.

A drawback of this algorithm is that we need to know the variance of the noise $s^2$, or at least have a good estimate.
In practice, we might be able to obtain such an estimate, but ideally our algorithm would work without knowing $s^2$.
By extending our algorithm, we obtain the following result:
\begin{theorem}[informal]
There is an algorithm \textsc{BucketGreedyMerge}, which, given $\vec{X}$ (of rank $r$), $\vec{y}$, and a target number of pieces $k$, runs in time $O(n d^2 \log n)$ and outputs an $O(k \log n)$-piecewise linear function $\fhat$ so that with probability at least $0.99$, we have
\[
  \MSE (\fhat) \; \leq \; O\left( \sigma^2 \frac{kr \log n}{n} + \sigma \sqrt{\frac{k}{n}} \log n \right) \; .
\]
\end{theorem}

At a high level, there are two fundamental changes to the algorithm: first, instead of merging with respect to the sum squared error of the least squares fit regularized by a term depending on $s^2$, we instead merge with respect to the average error the least squares fit incurs within the current interval.
The second change is more substantial: instead of finding the $O(k)$ candidates with largest error and merging the rest, we now split the candidates into $\log n$ buckets based on the lengths of the candidate intervals.
In this scheme, bucket $\alpha$ contains all candidates with length between $2^\alpha$ and $2^{\alpha + 1}$, for $\alpha = 0, \ldots, \log n - 1$.
Then we find the $k + 1$ candidates with largest error within each bucket and merge the remaining candidate intervals.
We continue this process until we are left with $O(k \log n)$ buckets.
%Intuitively, this bucketing allows us to control the variance of the noise without knowing $s^2$ because all candidate intervals have roughly the same length.

A potential disadvantage of our algorithms above is that they produce $O(k)$ or $O(k \log n)$ pieces, respectively.
In order to address this issue, we also provide a postprocessing algorithm that converts the output of any of our algorithms and decreases the number of pieces down to $2k  + 1$ while preserving the statistical guarantees above.
The guarantee of this postprocessing algorithm is as follows.
\begin{theorem}[informal]
There is an algorithm \textsc{Postprocessing} that takes as input the output of either $\textsc{GreedyMerge}$ or $\textsc{BucketGreedyMerge}$ together with a target number of pieces $k$, runs in time $O\left( k^3 d^2 \log n\right)$, and outputs a $(2k + 1)$-piecewise linear function $\fhat^p$ so that with probability at least $0.99$, we have
\[
  \MSE (\fhat^p) \; \leq \; O\left(\sigma^2 \frac{kr}{n} + \sigma \sqrt{\frac{k}{n}} \log n \right) \; .
\]
\end{theorem}
Qualitatively, an important aspect this algorithm is that its running time depends only logarithmically on $n$.
In practice, we expect $k$ to be much smaller than $n$, and hence the running time of this postprocessing step will usually be dominated by the running time of the piecewise linear fitting algorithm run before it.

In this document, we only give the formal pseudo code and proofs for \textsc{GreedyMerge}.
We refer the reader to the full version for more details.

\subsection{Comparison to prior work}
\label{sec:prior}

\paragraph{Dynamic programming.}
Previous work on segmented regression with statistical guarantees ~\cite{BP98, YP13} relies heavily on dynamic programming-style algorithms to find the $k$-piecewise linear least-squares estimator.
Somewhat surprisingly, we are not aware of any work which explicitly gives the best possible running time and statistical guarantee for this algorithm.
For completeness,  we prove the following result \newjd{(Theorem~\ref{thm:inf-DP}), which we believe to be folklore. The techniques used in its proof will also be useful for us later.}
\begin{theorem}[informal]
\label{thm:inf-DP}
The exact dynamic program runs in time $O(n^2 (d^2 + k ))$ and outputs an $k$-piecewise linear estimator $\fhat$ so that with probability at least $0.99$ we have  $\MSE(\fhat) \; \leq \; O\left( \sigma^2 \frac{kr}{n} \right)$.
\end{theorem}
We now compare our guarantees with those of the DP.
The main advantage of our approaches is computational efficiency -- our algorithm runs in linear time, while the running time of the DP has a quadratic dependence on $n$.
While our statistical rate of convergence is slower, we are able to achieve the same MSE as the DP in asymptotically less time if enough samples are available.

For instance, suppose we wish to obtain a MSE of $\eta$ with a $k$-piecewise linear function, and suppose for simplicity that $d = O(1)$ so that $r = O(1)$ as well.
Then Theorem \ref{thm:inf-DP} tells us that the DP requires $n = k / \eta$ samples and runs in time $O(k^3 / \eta^2)$.
On the other hand, Theorem \ref{thm:inf-greedy} tells us that \textsc{GreedyMerging} requires $n = \Otilde (k / \eta^2)$ samples and thus runs in time $\Otilde(k / \eta^2)$.
For non-trivial values of $k$, this is a significant improvement in time complexity.

This gap also manifests itself strongly in our experiments (see Section \ref{sec:experiments}).
When given the same number of samples, our MSE is a factor of 2-4 times worse than that achieved by the DP, but our algorithm is about $1,000$ times faster already for  $10^4$ data points.
%In fact, it quickly grew impractical to run the DP for more data points, and so we could not get comparisons much further beyond this many data points.
When more samples are available for our algorithm, it achieves the same MSE as the DP about $100$ times faster.

\paragraph{Histogram Approximation}
Our results build upon the techniques of \cite{ADHLS15}, who consider the problem of \emph{histogram approximation}.
Indeed, without too much work it is possible to convert their algorithm to our regression setting, but the resulting guarantee is not statistically meaningful (see the full version for a more detailed discussion).
To overcome this difficulty, we propose a merging algorithm based on a new merging error measure.
Utilizing more sophisticated proof techniques than in \cite{ADHLS15}, we show that our new algorithm has good statistical guarantees in the regression setting.

\subsection{Mathematical Preliminaries}
\paragraph{Tail bounds} We will require the following tail bound on deviations of squares of sub-Gaussian random variables.
We defer the proof to the supplementary material.
\begin{corollary}
\label{cor:unif-err-bound}
Fix $\delta > 0$ and let $\epsilon_1, \ldots, \epsilon_n$ be as in~\eqref{eq:model}.
Recall that $s = \EE [\epsilon_i^2]$.
Then, with probability $1 - \delta$, we have that simultaneously for all intervals $I \subseteq [n]$ the following inequality holds:
\begin{equation}
\label{eq:unif-err-bound}
 \left| \sum_{i \in I} \epsilon_i^2 - s^2 |I| \right| \; \leq \; O(\sigma^2 \cdot \log (n / \delta)) \sqrt{|I|} \; .
 \end{equation}
\end{corollary}

\paragraph{Linear regression.}
Our analysis builds on the classical results for fixed design linear regression.
In linear regression, the generative model is exactly of the form described in \eqref{eq:model}, except that $f$ is restricted to be a $1$-piecewise linear function (as opposed to a $k$-piecewise linear function), i.e., $f(\vec{x}) = \langle \vec{\theta}^\ast, \vec{x} \rangle$ for some unknown $\vec{\theta}^\ast$.

The problem of linear regression is very well understood, and the asymptotically best estimator is known to be the \emph{least-squares} estimator.
\begin{definition}
Given $\vec{x}_1, \ldots, \vec{x}_n$ and $y_1, \ldots, y_n$, the \emph{least squares estimator} $\fls$ is defined to be the linear function which minimizes $\sum_{i = 1}^n (y_i - f(\vec{x}_i))^2$ over all linear functions $f$.
For any interval $I$, we let $\fls_I$ denote the least squares estimator for the data points restricted to $I$, i.e. for the data pairs $\{(\vec{x}_i, y_i) \}_{i \in I}$.
We also let \textsc{LeastSquares} (\vec{X}, \vec{y}, I) denote an algorithm which solves linear least squares for these data points, i.e., which outputs the coefficients of the linear least squares fit for these points.
\end{definition}
Following our previous definitions, we let $\vecfls \in \R^n$ denote the vector whose $i$-th coordinate is $\fls(\vec{x}_i)$, and similarly for any $I \subseteq [n]$ we let $\vecfls_I \in \R^{|I|}$ denote the vector whose $i$-th coordinate for $i \in I$ is $\fls_I (\vec{x}_i)$.
The following error rate is known for the least-squares estimator:
\begin{fact}
\label{thm:LSrate}
Let $\vec{x}_1, \ldots, \vec{x}_n$ and $y_1, \ldots, y_n$ be generated as in~\eqref{eq:model}, where $f$ is a linear function. Let $\fls (x)$ be the least squares estimator. Then,
\[\EE \left[ \MSE (\fls) \right] = O \left( \sigma^2 \frac{r}{n} \right) \; .\]
Moreover, with probability $1 - \delta$, we have
\[\MSE (\fls) = O\left( \sigma^2 \, \frac{r + \log 1 / \delta}{n} \right) \; . \]
\end{fact}

Fact \ref{thm:LSrate} can be proved with the following lemma, which we also use in our analysis.
The lemma bounds the correlation of a random vector with any fixed $r$-dimensional subspace:
\begin{lemma}[c.f. proof of Theorem 2.2 in \cite{Rig15}]
\label{lem:incoherence}
Fix $\delta > 0$.
Let $\epsilon_1, \ldots, \epsilon_n$ be i.i.d.\ sub-Gaussian random variables with variance proxy $\sigma^2$.
Let $\vec{\epsilon} = (\epsilon_1, \ldots, \epsilon_n)$, and let $S$ be a fixed $r$-dimensional affine subspace of $\R^n$.
Then, with probability $1 - \delta$, we have
\[\sup_{\vec{v} \in S \setminus \{0\}} \frac{| \vec{v}^T \vec{\epsilon} |}{\| \vec{v} \|} \; \leq \; O\left(\sigma \sqrt{r + \log (1 / \delta})\right) \; . \]
\end{lemma}

This lemma also yields the two following consequences.
The first corollary bounds the correlation between sub-Gaussian random noise and any linear function on any interval (see the full paper for proofs):
\begin{corollary}
\label{cor:int-incoherence}
Fix $\delta > 0$ and $\vec{v} \in \R^n$.
Let $\vec{\epsilon} = (\epsilon_1, \ldots, \epsilon_n)$ be as in Lemma \ref{lem:incoherence}.
Then with probability at least $1 - \delta$, we have that for all intervals $I$, and for all non-zero linear functions $f: \R^d \to \R$, 
\[
  \frac{|\langle \vec{\epsilon}^I, \vec{f}_I + \vec{v}_I \rangle|}{ \| \vec{f}_I + \vec{v}_I \|} \; \leq \; O(\sigma \sqrt{r + \log (n / \delta)}) \; .
\]
\end{corollary}

\begin{corollary}
\label{cor:sim-incoherence}
Fix $\delta > 0$ and $\vec{v} \in \R^n$.
Let $\vec{\epsilon}$ be as in Lemma \ref{lem:incoherence}.
Then with probability at least $1 - \delta$, we have
\[
  \sup_{f \in \mathcal{L}_k} \frac{\left| \langle \vec{\epsilon}, \vec{f}_I+ \vec{v}_I \rangle \right| }{\| \vec{f}_I + \vec{v}_I \|}  \; \leq \; O \left( \sigma \sqrt{k r + k \log \frac{n}{\delta}} \right) \; .
\]
\end{corollary}

These bounds also imply the following statement, which we will need later. 
We defer the proof to the supplementary material.

\begin{lemma}
\label{lem:flat}
Fix $\delta > 0$.
Then with probability $1 - \delta$ we have the following:
for all disjoint sets of $k$ intervals $I_1, \ldots, I_k$ of $[n]$ so that $f$ is flat on each $I_\ell$, the following inequality holds:
\[
  \sum_{\ell = 1}^k \norm{\vecfLS_{I_\ell} - \vec{f}_{I_\ell}}^2 \; \leq \; O (\sigma^2 \, k (r + \log (n / \delta))) \; .
\]
\end{lemma}


